Sync-Switch: Hybrid Parameter Synchronization for Distributed Deep Learning

Stochastic Gradient Descent (SGD) has become the de facto way to train deep neural networks in distributed clusters. A critical factor in determining the training throughput and model accuracy is the choice of the parameter synchronization protocol. For example, while Bulk Synchronous Parallel (BSP) often achieves better converged accuracy, the corresponding training throughput can be negatively impacted by stragglers. In contrast, Asynchronous Parallel (ASP) can have higher throughput, but its convergence and accuracy can be impacted by stale gradients. To improve the performance of synchronization protocol, recent work often focuses on designing new protocols with a heavy reliance on hard-to-tune hyper-parameters. In this paper, we design a hybrid synchronization approach that exploits the benefits of both BSP and ASP, i.e., reducing training time while simultaneously maintaining the converged accuracy. Based on extensive empirical profiling, we devise a collection of adaptive policies that determine how and when to switch between synchronization protocols. Our policies include both offline ones that target recurring jobs and online ones for handling transient stragglers. We implement the proposed policies in a prototype system, called Sync-Switch, on top of TensorFlow, and evaluate the training performance with popular deep learning models and datasets. Our experiments show that Sync-Switch achieves up to 5.13X throughput speedup and similar converged accuracy when comparing to BSP. Further, we observe that Sync-Switch achieves 3.8% higher converged accuracy with just 1.23X the training time compared to training with ASP. Moreover, Sync-Switch can be used in settings when training with ASP leads to divergence errors. Sync-Switch achieves all of these benefits with very low overhead, e.g., the framework overhead can be as low as 1.7% of the total training time.

==> latex-tabs/exp_summary_speedup.tex <==
% \begin{table*}[t]
% \centering
% \resizebox{\textwidth}{!}{\begin{tabular}{ccc|c|c|c|c}
% \hline
% \multicolumn{3}{c|}{Exp. Setup} & \multicolumn{2}{c|}{Throughput Speedup Over} & \multicolumn{2}{c|}{TTA Speedup Over} \\ \hline
% Dataset    & Model    & Cluster & ASP                   & BSP                  & ASP              & BSP                \\ \hline
% Cifar-10   & ResNet32 & 8       & 0.78X                 & 5.13X                & NA               & 3.99X              \\
% Cifar-100  & ResNet50 & 8       & 0.89X                 & 1.66X                & NA               & 1.60X              \\
% Cifar-10   & ResNet32 & 16      & NA                    & 1.87X                & NA               & 1.08X              \\ \hline
% \end{tabular}}
% \label{table:eval_speedup_analysis}
% \caption{The speedup of solutions found by \sysname compared to the baselines on three selected metrics
% \tian{merge with the Table~\ref{table:exp_summary_policies}}
% }
% \end{table*}

==> section/background.tex <==
\section{Background}
\label{sec:background}

In this section, we first provide a brief overview about distributed training in Section~\ref{subsec:dll}. We then provide important premise of this work with the description on existing parallel synchronization protocols (Section~\ref{subsec:protocols}) and adaptive and dynamic training (Section~\ref{subsec:adaptive_training}).

\subsection{Distributed Deep Learning}
\label{subsec:dll}

% In this work, we target \emph{distributed deep learning} where multiple computing nodes (also referred to as \emph{workers}) with GPU devices are working together to train a deep neural network by communicating via network. We focus on the more popular approach \emph{data parallelism}, where the training data or mini-batches are partitioned and offloaded to the computing nodes, instead the \emph{model parallelism}. When training with data parallelism, each node will train on the complete neural network with a subset of data to update the model parameters. To facilitate the exchange of model parameters, a logical role of parameter servers (PSs) was separated out from the computing nodes and serves as the hub for communicating with computing nodes. There are various ways to setup the PS, e.g,. as a centralized node or being distributed onto several nodes, or running as a dedicated node or collocating with computing nodes.

In this work, we target \emph{distributed deep learning} where multiple computing nodes (also referred to as \emph{workers}) with GPU devices are working together to train a deep neural network by communicating via network. We focus on the more popular approach \emph{data parallelism}, where the training data or mini-batches are partitioned and offloaded to the workers, instead the \emph{model parallelism}. When training with data parallelism, each node will train on the complete neural network with a subset of data to update the model parameters. 
To facilitate the exchange of model parameters, a logical role of parameter servers (PSs) are setup as the hub for communicating with computing nodes. In this work, we study the popular scenarios where the parameter servers are collocated with workers (therefore being distributed), because of less network communication.

% In this work, we study the scenarios where the parameter servers are collocated with computing works (therefore being distributed), which we refer to as \emph{collocated PSs}.
% We chose this architecture due to its increasing popularity, e.g., supported by major frameworks\tian{?} and investigated by prior work\tian{add citations!}, and its numerous benefits. First, collocating workers and parameter servers can alleviate the network communication bottleneck problem commonly observed in dedicated PS \tian{needs citation!} 
% Second, collocated PSs can save operation cost, especially in the cloud environment, as there is no need for renting additional cloud servers to serve as dedicated PSs. \tian{citations}
% Third, as collocated PSs share more similarities to other popular distributed training architectures, such as ring-allreduce, it lowers the barrier for adapting our work to other training architectures. \tian{I think we can condense the benefits of collocated PSs if space is limited.}


When using the collocated PSs, one needs to divide the model parameters into different shards, each shard managed by one PS instance.
%
\tian{Write a sentence about sharding and cite techniques to generate shards and what we use.}
% TG: replace this sentence with Lijie's suggestions.
\tian{REPLACE for more detailed version. During the training, the workers communicate with all PSs in each training iteration: pulling model parameters to compute gradients by working on the database and pushing the newly computed gradients. The PSs then update the model parameters based on the collected gradients.}
%
% \tian{Needs to describe how different parameter servers communicate with each other, what protocols.}





\subsection{Distributed Parameter Synchronization Protocols}
\label{subsec:protocols}

%%%

\begin{figure}[t]
    \centering
    
    \includegraphics[width=\textwidth]{img/BSP-ASP-SGD.pdf}
    
    \caption{Two popular distributed parameter synchronization protocols. When using BSP, PSs employ a barrier for gradient collection and only start to update parameters once all gradients are aggregated. In contrast, when using ASP, individual worker pushes gradients and pulls parameters at their own paces.}
    \label{fig:distributed_synchronization_protocols}
\end{figure}
%%%

% \begin{figure}[t]
%     \centering
%     \begin{subfigure}[t]{0.47\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/BSP-SGD.pdf}
%         \caption{Bulk Synchronous Parallel.
%         }
%         \label{fig:bsp}
%     \end{subfigure}
%     \qquad
%     \begin{subfigure}[t]{0.47\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/ASP-SGD.pdf}
%         \caption{Asynchronous Parallel.
%         }
%         \label{fig:asp}
%     \end{subfigure}
%     \caption{Two popular distributed parameter synchronization protocols. When using BSP, PSs employ a barrier for gradient collection and only start to update parameters once all gradients are aggregated. In contrast, when using ASP, individual worker pushes gradients and pulls parameters at their own paces.
%     \Lijie{I'm going to re-draw this figure.}} 
%     \label{fig:distributed_synchronization_protocols}
% \end{figure}



In distributed deep learning, synchronization and coordination of worker progress (i.e., gradient computation) is achieved by \emph{distributed parameter synchronization protocols} \tian{add citations}. There are two popular protocols:
\emph{Bulk Synchronous Parallel} (BSP) and \emph{Asynchronous Parallel} (ASP) that differ in their horizontal scalability, sensitivity to stragglers, and converged test accuracy. 

\Lijie{As shown in Figure~\ref{fig:distributed_synchronization_protocols}. The parameter of neural network $w$ is a large vector distributed into parameter servers. Data $d$ is divided to $m$ mini-batches, and each mini-batch $d_i$ is distributed into $n$ workers. Thus, each worker $j$ has a part of data as $d_{ij}$. Each worker $j$ computes gradients $g{ij} = bp(d_{ij}, w_i)$. The PSs collect all the $g_{ij}$ from all the workers, and compute new parameter $w$, and then distribute $w$ into workers for next mini-batch. This is synchronous update, because the PSs need to wait for getting $g_{ij}$ from all the workers and then perform update on $w$. To reduce wait time, the framework also support asynchronous update, i.e., the $w$ is updated to $w$ when getting a $g_{ij}$ from a worker. The P-new is broadcast to workers at some points XXX. However, asynchronous update may force the workers use stale parameters}.

BSP, as shown in Figure~\ref{fig:bsp} is a deterministic scheme where workers perform a parallel computation phase followed by a synchronization phase where the gradients are aggregated at a barrier. The model parameters then update according to this aggregated set of gradients. This method ensures that all workers are working on the same iteration of model parameters, and prevents any worker from proceeding to the next iteration before others. 
% 
Furthermore, the effects of the current computation are not made
visible to other workers until the barrier has been reached. This guarantees the method to be equivalent to a true mini-batch stochastic gradient descent algorithm, with its effective batch size equal to the sum of the sizes of the mini-batch on all the workers, thus ensuring the correctness of the parallel computation~\cite{chen2016revisiting}.
%
The main drawback of BSP is that it is greatly affected by the presence of straggler
nodes. Since the workers need to wait for all updates to finish and be collected
at the barrier, the faster workers all remain idle while waiting for the
stragglers. This drastically limits the training performance of the whole
training cluster. Generally speaking, BSP offers high computation accuracy but
suffers from poor efficiency in unfavorable environments.

ASP, as shown in Figure~\ref{fig:asp}, allows computations to execute in parallel as fast as possible by running workers completely asynchronously. Each worker individually pulls parameters and pushes new gradients for update to the parameter server. In homogeneous environments (e.g. data centers), wherein the
workers have similar configurations, ASP enables fast convergence because it
permits the highest iteration throughput. Typically, near-linear speed-ups can
be achieved by adding more computation resources, and the scaling bottleneck usually comes from bandwidth among the computing nodes. On the other hand, such asynchronous computation causes delayed updates: updates calculated on an old model parameter state which should
have been applied earlier but were not. These are called stale gradients, and applying them introduces noise and error
into the computation. Consequently, ASP suffers from decreased iteration quality
and may even diverge in unfavorable environments. Overall, ASP offers excellent
speed-ups in convergence but has a greater risk of diverging especially in a
heterogeneous context. 

%%%
\begin{figure}[t!]
    \centering
        \includegraphics[width=0.4\textwidth]{img/motivation_straggler.pdf}
        \caption{\textbf{Straggler impact on ASP and BSP}\shijian{We might also show the converged accuracy?}
        \tian{we should! Also, where are the error bars? \2 Also it can be confusing to see that the normalized training time are the same for BSP and ASP without straggler? Need to think about alternative ways to plot. \3 Maybe we should add an accuracy impact for ASP as the cluster size grows (for staleness) as we will have the data handy...} }
        \label{fig:strag}
\end{figure}
%%%

In summary, ASP and BSP have advantages and disadvantages weighing on different priorities in training: ASP for converged accuracy and BSP for training throughput. Traditionally, the method for synchronization is determined at the start of training, and takes effect until the neural network has been fully trained. 
We conducted a small-scale empirical study with training clusters of 4-workers and 1 GPU each training ResNet32 on Cifar-10 to highlight the key factors that impact the training performance using BSP and ASP. Figure~\ref{fig:strag} shows that stragglers in the training cluster severely impact the total training time of BSP, \tian{with up to XX times slowdown compared to using ASP.}
%
\tian{either we need to mention we omit the accuracy comparison because they are not interesting or we need to add in the accuracy comparison.}
Our observations align with recent work \tian{citations} and serve as one of the key insights for improving the performance of distributed deep learning (see Section~\ref{sec:motivation} for additional details.)


\subsection{Adaptive Training Configurations}
\label{subsec:adaptive_training}

\tian{Meta comments: it seems that a lot of paragraphs written in this section are written without explicitly citing prior work... which needs to be rectified by adding proper citations...}

Recent studies \tian{add citations} have started looking at changing distributed training configurations either based on training progress such as gradient staleness or external factors, e.g., network communication, which we refer to as \emph{adaptive training}. Depending on the knob being adjusted, we categorize existing adaptive training work into three types. Our work expands prior work and introduces a new category on adaptive distributed parameter synchronization protocols.

The first knob is \emph{batch size}, \tian{please look for alternative definition}. 
%
\tian{needs to provide the intuition of why changing batch size can be useful!} 
Recent studies such as \tian{XX and YY} explore the benefits of changing the batch size over time \tian{based on what policies?}. 
%
The second knob is \emph{learning rate}, a hyper-parameter that controls how much to change the model in response to the estimated error each time the model weights are updated. Choosing the learning rate is challenging as a value too small may result in a long training process that could get stuck, whereas a value too large may result in learning a sub-optimal set of weights too fast or an unstable training process. Therefore the learning rate is usually set to be changing overtime. Typically, learning rate decays in value as the training goes on. And the timing for decay is usually pre-determined using some functions such as step/piecewise or cosine. \tian{please add citations for adaptive and dynamic learning rates!}
%
The last popular knob is \emph{cluster size}, which defines the number of workers in the training cluster. Previous studies have shown that cluster size might negatively impact the training performance in terms of convergence \tian{add citations.}. However, recent studies~\cite{lin2019dynamic,Or_undated-nh} have shown an increasing amount of interest in dynamically adding or striping away resources from training clusters during training \tian{provide a sentence about how?!!!}. This was mainly done to accommodate for resource scheduling and availability issues, and improve resource utilization.


\tian{Please move this to the related work section; this feels out of place.}
Until very recently, there have been a surge of research interest for adjusting how the distributed parameter synchronization protocols work, as the fourth knob. 
Such examples include Stale Synchronous Parallel (SSP), Dynamic Stale Synchronous Parallel (DSSP),
Probabilistic Synchronous Parallel~\cite{wang2017probabilistic}, Elastic Bulk Synchronous Parallel
~\cite{zhao2019elastic}. \tian{add citations! In addtion to list all these names, it will be much more interesting to summarize the key ideas of how they work!} These studies are either based on BSP or ASP, focusing on solving the drawbacks of the method. However, they still strike a balanced trade-off between converged accuracy and training speed, and cannot achieve both the speed of ASP and the accuracy of BSP. Additionally, some of these work introduced new user-controlled hyper-parameters. These hyper-parameters needs to be repeatedly tuned to find an optimal value, which could be difficult and impractical for the deep learning practitioners. Moreover, these emerging synchronization protocols are often used in conjunction with static training configurations and will remain the same for the entire training duration. 

==> section/design.tex <==
\section{Design}
\label{sec:design}

In this section, we propose the method of switching the synchronization dynamically based on different switching policies. We will go over several heuristics that can exploit the potential of this method, and some associated trade-offs and overheads to consider. We highlight several design choices we made for switching SGD algorithms to optimize desired training performance.

\tian{we should add a diagram to provide the readers an intuitive understanding regarding how the switching policy works, e.g., a concrete example that triggers switching.}

We focus on answering the following questions.
First, how many switching is needed to achieve desirable training performance? As current training frameworks do not support seamless configuration changes while the training is ongoing, switching might increase total training time.
Second, when does it make sense to switch from BSP to ASP or vice versa?
%First, when does it make sense to switch from BSP to ASP and vice versa? As
%current training frameworks do not support seamless configuration changes while
%the training is ongoing, switching might increase total training.
%Second, as our decisions are driven by the performance metrics, we also need to
%decide the frequency to collect and analyze these performance metrics as well.
%Intuitively, a smaller interval allows us to quickly react to the changes in the
%training environment but imposes higher logging overhead.

\paragraph{Goals and assumptions for SGD switching}

\shijian{Goals and assumptions should be more suitable for problem statement. Some key design principles and intuition could be here}

In this work, we assume the following for the input workload: \tian{Paper structure comments: The assumptions should be described in the problem statement section already.}

\begin{itemize}
\item{The model to be trained and the training dataset has been seen before. This scenario is common for recurring deep learning jobs or other jobs such as fine-tuning.} \tian{What does fine-tuning refer to? Don't assume reviewers have extensive knowledge in general.}
\item{The amount of training is given, which means that we know how many steps/epochs the user wants to train.} \tian{Are these all the assumptions we are making? How about the hyperparameters that were mentioned below?}
\end{itemize}

We preserve the majority of the hyperparameters and settings provided in the beginning throughout the training, even when switching SGDs. By training on the same workload but using SGD switching we aim to provide model test accuracy as high as possible, close or on par with the level of static BSP, while greatly reducing the total training time. \tian{What does static BSP mean? Meta comment: it is generally safer to define a term the very first time you introduce it. 2. Another important aspect when writing design section is to set the correct expectations for the Evaluation section. We want to gradually introduce the baseline and related work to the reviewers before the evaluation section, and then present a comprehensive evaluation.}

\subsection{The ordering of SGD algorithms}

The aim of our method is to achieve a testing error that is as low as when training exclusively with BSP, while still benefiting from (nearly) the  same  linear speedup in the per-epoch computation time afforded by ASP. %which is roughly linear in the number of workers.
%
Since we care only about minimizing the testing error, our ultimate goal is to minimize the population loss--the loss value for the population distribution from which our dataset was sampled-- even if this does not lead to the lowest possible training loss value.
%
We argue here that using BSP in the earlier epochs and then switching to ASP can allow us to simultaneously accomplish both the goals of minimizing the population loss and improving the per-epoch computation time.

\tian{Is the argument regarding learning rate generalizable? Are we indicating that the common learning rate schedules often decay learning rate as the training goes on?}
%
First, we note that the steps taken by momentum-SGD earlier in the training are much larger than those taken later in the training.  This is because, (1)  at earlier epochs  the gradient tends to have a much larger magnitude, since it is further from a local minimum point  than at later epochs and (2)  many state-of-the-art results use a decaying learning rate schedule, where the learning rate is much larger at earlier epochs than at later epochs.

Next, we argue (in Section \ref{sec_loss_landscape}) that at coarser scales correspoding to the large steps taken by the algorithm earlier in the training, the landscape of the population loss function resembles that of the training loss.
%
On the other hand, past empirical work \cite{kleinberg2018alternative, hochreiter1995simplifying, hochreiter1997flat, keskar2016large, smith2018bayesian, chaudhari2019entropy} suggests that at finer scales corresponding to the smaller steps taken later in the training, the landscape of the population loss is much smoother than that of the training loss. 
%


%
 Finally, we note that while stale gradients may be ineffective very early in the training when larger steps are taken by the algorithm, stale gradients can be used to effectively minimize the population loss later in the training, since the landscape of the population loss is much smoother on a finer scale corresponding to the smaller steps taken by the algorithm later in the training.
 This is because, at later epochs, the gradient of the population loss does not change as quickly each time the algorithm takes a step, which means that stale gradients  may still be able to provide useful information about the gradient of the population loss at the current point even though the stale gradients were computed at previous (but nearby) points.  This suggests that ASP can effectively minimize the training loss if it is used at later epochs.

On the other hand, at very early epochs, when the algorithm takes much larger steps, the gradient of the population loss may change very quickly at each step.  This means that stale gradients may not provide much information about the value of the gradient at the current point.  This suggests using BSP early in the training, and then switching to ASP at a later epoch. This hypothesis is supported by our emperical results, which show that using BSP at earlier epochs and switching to ASP at later epochs   allows one to obtain a testing
error which is as low as in experiments using BSP during the entire training.

\begin{figure}[t!]
    \centering
    \begin{subfigure}[t]{0.2\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/cartoon_BSP.pdf}
        \caption{\textbf{BSP.}}
        \label{fig:cartoon_BSP}
    \end{subfigure}
    \,
    \,
    \,
    %
    \begin{subfigure}[t]{0.2\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/cartoon_ASP.pdf}
        \caption{\textbf{ASP.}}
        \label{fig:cartoon_ASP}
    \end{subfigure}
  %
        \begin{subfigure}[t]{0.2\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/cartoon_BSP_to_ASP.pdf}
        \caption{\textbf{Switching, BSP to ASP.}}
        \label{fig:cartoon_BSP_to_ASP}
    \end{subfigure}
    %
    \,
    \,
    \,
          \begin{subfigure}[t]{0.2\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/cartoon_ASP_to_BSP.pdf}
        \caption{\textbf{Switching, ASP to BSP.}}
        \label{fig:cartoon_ASP_to_BSP}
    \end{subfigure}
    %
    \caption{Illustrations of various combinations of BSP and ASP on a simple smooth loss function (blue level sets). All algorithms have larger step sizes in earlier epochs (due to larger learning rates and larger gradient magnitudes earlier in the training).  This means that, in earlier epochs, the gradient changes quickly at each step and stale gradients (red) are much less reliable than non-stale gradients (black).  Thus algorithms which use ASP earlier in the training may have a difficult time settling into a local minimum region where the gradient is small (b, d).  This is true even if one switches from ASP to BSP (d) as the algorithm may get stuck in a saddle point once the learning rate has decayed, causing it to take a long time to escape the saddle point.  In contrast, if one only uses stale gradients at later epochs once the algorithm is closer to a minimum point, the stale gradients will be low-bias estimates for the true gradient and will still allow the algorithm to reach the minimum point (c).}
\end{figure}





\begin{figure}[t!]
    \centering
    \begin{subfigure}[t]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/Cartoon_training_loss_BSP.pdf}
        \caption{\textbf{BSP.}}
        \label{fig:cartoon_BSP_training_loss}
    \end{subfigure}
    \,
    \,
    \,
    %
    \begin{subfigure}[t]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/Cartoon_training_loss_BSP_ASP.pdf}
        \caption{\textbf{BSP to ASP.}}
        \label{fig:cartoon_ASP_training_loss}
    \end{subfigure}
    %
    \caption{The training loss (greed solind curve) is not as smooth as the population loss  (blue dashed curve).  Thus, the stale gradients used by our algorithm (b) do not allow it to find the minimum of the training loss as well as BSP (a).  However, it is still able to find the a point which minimizes the population loss as well as BSP.}
\end{figure}

\begin{remark}[Can switching from BSP to ASP also minimize the training loss?]
%
In the previous discussion we have used the fact that the population loss is oftentimes much smoother than the training loss.
%
  For this reason, even if one only uses stale gradients later in the training when the algorithm takes smaller step sizes, the gradient of the training loss may still change rapidly at each step of the algorithm despite the fact that the gradient of the population loss may not be changing as quickly.
%
This suggests that, while using ASP later in the training may allow one to effectively minimize the population loss, it may still not allow one to minimize the training loss.
%
This is exactly what we observe in our experiments: while switching from ASP to BSP allows one to minimize the testing error (and hence the population loss) as effectively as using BSP alone, the training loss remains much higher than in experiments where BSP alone is used.

\end{remark} 

\subsubsection{Population loss landscape at different scales}\label{sec_loss_landscape}
 There is much empirical and heuristic evidence that the  population loss is in fact much smoother than the training loss. 
%
 For instance, it has been observed that sharp local minima of the training loss-- minima where the training loss  is only low in a small region near the  minimum point-- oftentimes do not correspond to a low test loss \cite{hochreiter1995simplifying, hochreiter1997flat, keskar2016large, smith2018bayesian, chaudhari2019entropy}.
%
  On the other hand, ``flat"  local minima of the training loss-- local minima where the training loss remains low in a wide region containing the local  minimum point-- in many cases also minimize the test loss.
%
Moreover, it has recently been shown that minimizing a ``smoothed" version
of the training loss can lead to a test error that is as low, or oftentimes
even lower, than if one were to minimize the training loss itself. 
%
Here the smoothed loss function is the convolution of the loss function with
the distribution of the batch gradient noise (the variance of the noise depends
on the batch size) \cite{kleinberg2018alternative}.

This evidence suggests that  the population loss is  much smoother than the training loss, and is in fact closer to a  ``smoothed" version of the training loss convolved with  a the distribution of the batch gradient noise rather than the original training loss.  This suggest that our population
loss will have a lanscape that is smooth at  a finer scale on the order of the learning rate used later in the training.  On the other hand, at coarser scales--on the order of the large learning rate used earlier in the training--we expect the landscape of the population loss to be much closer to the training loss. In other words, earlier in the training, when a large step size is used, the change in the training loss and population loss at each step should be roughly the same, and the ratio of the change in the population loss to the change in  training loss should be close to 1.  Later in the training, when a much smaller learning rate is used, this ratio could be very far from 1.

\subsubsection{Dynamic switching criterion}
%
One can view both the stale gradients used in ASP and the non-stale gradients used in ASP as stochastic estimates for the gradient of the population loss.
%
Since both stale and non-stale  gradients are computed using training data, their means (conditional on the training data), are not unbiased estimates of the population loss gradient.
%
Rather, the conditional mean of both the stale (ASP) gradients and non-stale (BSP) gradients differs from the population loss gradient by some error term.
%
The magnitude of this error for the BSP gradients is determined by the variance of the batch gradients.
%
For the ASP gradients, the error also depends on the magnitude of the difference between the non-stale gradient and the stale gradients.

We would like to switch from BSP to ASP when the error of the stale ASP gradients drops to a level where it is of roughly the same magnitude as the error of the non-stale BSP gradients.
%
To estimate the additional error we would incur by using stale (ASP) gradients, we will first compute the difference $\Delta_i = g_i - g_{i-k}$ 
between the batch gradient $g_i = \sum_{\xi \in \mathcal{B} \nabla L(x_i; \xi)}$ at the current step $x_i$ for some batch $\mathcal{B}$,   and the batch gradient   $g_{i-k} =  \sum_{\xi \in \mathcal{B}'} \nabla L(x_{i-1}; \xi)$ at a previous step $x_{i-k}$ computed with a different batch $\mathcal{B}'$, where the hyper-parameter $k$ represents the additional amount of time it takes the slowest worker to finish (in practice, you should use $k=1$).

Next, we would like to estimate the error of the non-stale (BSP) gradients in the direction $\Delta$; this error is can be estimated with the sample standard deviation
\begin{align}
\sigma_i & = \frac{1}{\sqrt{B}}\sqrt{ \frac{1}{B}\sum_{\xi \in \mathcal{B}} [\Delta_i^\top( \nabla L(x_i; \xi) - g_i)/ \|\Delta_i\|]^2}\\
&= \frac{1}{B\|\Delta_i\|} \sqrt{\sum_{\xi \in \mathcal{B}} [\Delta_i^\top( \nabla L(x_i; \xi) - g_i)]^2}  \\
\end{align}
When our estimate for the ASP error, $\|\Delta_i\|$, becomes small enough that it is comparable to our estimate for the BSP error, $\sigma_i$, we switch from BSP to ASP.
%
More specifically, we switch from BSP to ASP at the first time $i$ when $\|\Delta_i\|< c \sigma_i$, where the hyperparameter $c$ is some small constant greater than $1$ (or perhaps once this criterion is satisfied for some number $T$ steps in a row, where $T\in \mathbb{N}$ is another hyperparameter chosen by the user).


\subsubsection{Side effects of switching}

\tian{Why does this section belong here? They are not part of our deisgn; but instead, they are some practical limitations we should consider when designing the switching policy. The restoration overhead can be significantly avoided by rewriting part of TensorFlow (which we are not doing) while the training loss spike is currently being investigated by us. Bottomline, you need to make the distinction about three things: the world as it is, our proposed idea, and ways to evaluate the idea.}

We conducted the experiments using TensorFlow and Tensor2Tensor, which don't have native support for switching synchronization during training. Thus we emulated the switching process using checkpoint restoration. To emulate a switch from BSP to ASP, we first train the model with BSP and generate checkpoints at the designated steps. Then we restore the training session from these checkpoints using ASP.

As a result of the lack of support for a versatile training schema where the synchronization method can be switched on the fly. The training session needs to halt first, then a checkpoint needs to be generated, finally a new training session should be started with a different synchronization method. This will incur a non-negligible amount of overhead for training.

Training loss spike will occur when switching from BSP to ASP. Upon switching, training loss in all training sessions had an uptick. And the further it is into training, the greater the uptick. In other word, the smaller the loss value is, the bigger the uptick is going to be. \shijian{could put w28 1 to 4 img here in subplots to demostrate}

\subsection{Changing the training parameters between BSP and ASP}

\tian{Let us try to avoid using subsubsections if we can help it--- subsubsection makes the typesetting less asthetically pleasing. Instead, use the paragraph command.}

\tian{Meta comment: Most of what you wrote for this section is about what we did, without a number of important high-level descriptions, i.e., why do we need to use different training parameters (and what they are) after switching to ASP? What criterias are we using to measure the success?}


\subsubsection{Enhance training performance by tweaking learning rate}

We applied a constant scalar to base learning rate based on what distributed SGD is currently being used, based on previous study~\cite{goyal2017accurate} and common practice. For BSP we scale it up linearly to the number of workers, and for ASP we scale it down to the square root of the number of workers.

\subsubsection{Adjusting the momentum term to handle training loss spike}

Why do we care about the training loss spike if the metric to measure how good the training performs is converged test accuracy?

\begin{itemize}
\item{First, the training loss spike correlates to the test accuracy. Generally speaking, when properly trained (meaning no overfit or underfit), also depending on the complexity of the model and the dataset trained, the lower the training loss is, the higher the test accuracy will be}
\item{Second, although we focused on Cifar-10 and ResNet32 which are relatively simple workloads, thus making the earlier switching point feasible, in a different training scenario the switching point could come at a much later stage of training. The training loss spike, if not given enough room to recover, might lead to worse test accuracy for the designated training schedule}
\end{itemize}

As an important contribution to the paper, we observed the side effects of doing SGD switching under the limitation of current deep learning frameworks, and raised some potential solutions to solve them. \tian{Meta comments: generally speaking, all the solutions we will be described in the design section should have already been tested in a number of conditions---these solutions should not be referred to as "potential solutions". More concretely, we should only describe the momentum based solution in the design; but we can show a number of other intutive solutions including the batch size one as part of the evaluation and observations.} One major side effect when switching from BSP to ASP is the training loss spike.

After some empirical experiments, we found out that one potential cause is due to the disparity between batch sizes used before and after switching, as a result of changing the logic of the implementation. Our proposed solution is to (gradually) reduce batch size for BSP before switching, alongside with learning rate changes, to match that of the ASP local batch size.

However, the solution didn't work. Thus we look at another possible cause, the momentum. Due to the logic of restoration of training sessions, the momentum from BSP training session is carried over to the ASP session. Because the ASP training is usually behave slightly different than BSP, such as being more noisy, the momentum would potentially be a misfit and harm the training performance instead of helping it.

\shijian{w33\_1, w33\_2, w33\_3 momentum SGD update rules}

In the equation we have two variables $\mu$ and $v_t$ determining the value for the momentum term. $\mu$ is a constant scalar throughout training applied to the momentum value $v_t$ at time $t$, which is a transient vector values. To control the momentum term we could choose to adjust $v_t$, and this is equivalent to adjust $\mu$ by the same scalar for only one step. Thus it is better to adjust $\mu$

\tian{Meta comment: it is important to think about what the new world state is after the completing of our project. When writing a paper, it is less important to describe the various roads we took to arrive at the new state. It is more important to describe which road we took and why intutively this road will lead to a better state (which of course we will also need to have empirical results to backup in the eval section).}

\subsubsection{Preserving the training workload}

\tian{It is not clear what this subsection is supposed to convey.}

We conducted the experiments using TensorFlow and Tensor2Tensor, where the implementation logic for BSP and ASP has different views on the notion of batch size.

In BSP training, the batch size is global, seeing as an aggregated value to be distributed on the workers. However, in ASP training the batch size is treated as a local value specific to each worker.

Due to this batch size change in the training session from global to local, we did the following to preserve the consistency of the original learning rate schedule. We decay the learning rate at different steps, according to the workload processed into training, instead of the fixed steps of 32k and 48k. For example, for a split of 20\% BSP and 80\% ASP, since we have 8 workers, global batch size in BSP is 8X larger than local batch size in ASP. Thus we have BSP to train 1600 steps and ASP 51200 steps, with the total amount of images processed still $64000 * 128$. And we change the learning rate schedule to be \textit{[20800, 36800]} instead of \textit{[32000, 48000]} so that the learning rate still decays at the same amount of training workload.

Known parameters: training cluster size \textit{N}, total amount of workload \textit{W} (image wise), learning rate decay schedule [\textit{$W_1$}, \textit{$W_2$}], ASP batch size \textit{B}, BSP split \textit{$S_{bsp}$}. Note: We only need to know ASP batch size because BSP batch size is $B*N$. We only need to know BSP split because ASP split is $1-S_{bsp}$.

For BSP steps, we get the steps by $(W * S_{bsp}) / (B * N)$. Then we get ASP steps by $W / B - (W * S_{bsp}) / B$

Notice that for BSP training the training session sees all the input parameters from the perspective of BSP, thus step size etc. need to be scaled up. Once the training session switched to ASP, it is from the angle of ASP so no scaling is needed.

The total amount of steps is given by $(W * S_{bsp}) / (B * N) + W / B - (W * S_{bsp}) / B$

The first learning rate decay boundary can be calculated as $(W_1 / B) - (W * S_{bsp}) / B + (W * S_{bsp}) / (B * N)$

The second learning rate decay boundary is similarly given by $(W_2 / B) - (W * S_{bsp}) / B + (W * S_{bsp}) / (B * N)$

\begin{table*}[]
\centering
\begin{tabular}{|l|llll|}
\hline
Split \% (BSP-ASP) & BSP steps & ASP steps & Total steps & Learning rate schedule \\ \hline
0-100              & 0         & 64000     & 64000       & {[}32000, 48000{]}     \\
2-98               & 160       & 62720     & 62880       & {[}30880, 46880{]}     \\
4-96               & 320       & 61440     & 61760       & {[}29760, 45760{]}     \\
5-95               & 400       & 60800     & 61200       & {[}29200, 45200{]}     \\
10-90              & 800       & 57600     & 58400       & {[}26400, 42400{]}     \\
15-85              & 1200      & 54400     & 55600       & {[}23600, 39600{]}     \\
20-80              & 1600      & 51200     & 52800       & {[}20800, 36800{]}     \\
25-75              & 2000      & 48000     & 50000       & {[}18000, 34000{]}     \\
50-50              & 4000      & 32000     & 36000       & {[}4000, 20000{]}      \\
75-25              & 6000      & 16000     & 22000       & {[}4000, 6000{]}       \\
100-0              & 8000      & 0         & 8000        & {[}4000, 6000{]}       \\ \hline
\end{tabular}
\caption{Learning rate schedule scaling for our scenarios}
\label{tbl:learning_rate_schedule}
\end{table*}

\subsection{Switching Trade-offs and Overhead}

The basic idea of dynamic switching is to swap a synchronization method for another one mid-training, according to specific policies. These policies are based on different factors, both internal and external to the training process. In this work, we identify two potential key factors to build switching policies on.

\begin{itemize}
\item{Training loss. Training loss is the output value of the loss function used in training, after an iteration of forward propagation takes place. It is highly correlated to converged accuracy of the trained model. Because the convergence is the bottleneck for ASP, we use this factor as a metric to switch from ASP to BSP.}
\item{Training throughput. This factor is defined by how many examples(images) are being trained per second across all the workers. As this factor severely limits the training performance of BSP, we use it as a metric to switch from BSP to ASP.}
\end{itemize}

One thing to consider when switching synchronization method is the associated overhead. Currently, all major deep learning frameworks don't provide support for a versatile training schema where the synchronization method can be switched on the fly. The training session needs to halt first, then a checkpoint needs to be generated, finally a new training session should be started with a different synchronization method.

\subsection{Our Proposed Switching Policies}

Although the factors identified above serve as important points to consider for switching policies, they can not be used directly as metrics to arbitrate the triggering events for switching. The reason for this is two-fold:

\begin{itemize}
\item{We can't explicitly know the training throughput without conducting the training in the first place. This is especially true when we are facing novel neural networks, datasets, or training configurations.}
\item{Loss values differs greatly during training for different networks and training configurations. There's no unified standard to apply to myriad of different training scenarios.}
\end{itemize}

Therefore, we propose to use the \emph{delta} value of these two factors as metrics, denoted $\Delta_{throughput}$ and $\Delta_{loss}$. This way, we don't need knowledge about the training scenario a prior, and it is more generally applicable.

First we take a look at how we define the triggering point of $\Delta_{throughput}$. In the context of cloud-based deep learning, we found out through empirical study that the average fluctuation of training throughput is within the range of XX\%-YY\%. Thus when $XX\%<\Delta_{throughput}<YY\%$ and current synchronization method is BSP, we switch it to ASP.

Similarly, we define the triggering point of $\Delta_{loss}$ as \shijian{the
value is currently still being looked at. The gist is to make it more general,
and not network specific}.

\subsection{Sketch of Our Switching Policy}

\begin{algorithm}
\caption{Searching algorithm for optimal split}
\begin{algorithmic}
\STATE \textbf{Inputs:} Workload Split $S=100$,  Training efficiency $\beta=0$, $\alpha_{prev}=0$, Threshold $\tau=0.1$
\WHILE{$S=100$ \textbf{OR} $\beta > \beta_{prev}$}
\STATE $\beta_{prev}=\beta$
\STATE Train the model using hybrid of $BSP$ and $ASP$ with workload split of $S$ to get converged accuracy $\alpha$ and total training time $T$
\STATE $\beta = \alpha/T$
\IF{$\alpha >= \alpha_{prev}$ \textbf{OR} $|\alpha_{max} - \alpha| < \tau$}
\STATE $S=S/2$
\ELSE
\STATE $S=2*S$
\ENDIF
\STATE $\alpha_{prev} = \alpha$
\STATE $\alpha_{max} = MAX(\alpha, \alpha_{max})$
\ENDWHILE
\label{alg:binary}
\end{algorithmic}
\end{algorithm}

For a given training workload and cluster of $n$ servers, we will start the
training using BSP by default.
Assume we analyze whether switching between BSP and ASP might be beneficial for
the current workload every $\tau$ minutes, by estimating the remaining training
time $T_{bsp}$ and $T_{asp}$ with BSP and ASP, respectively.
Further, assume the average cluster training speed is $S_\tau$ and standard
deviation is $C_\tau$ between $[0, \tau]$, a worker is marked as a straggler if
its speed falls outside $\frac{S_\tau}{n} \pm \frac{C_\tau}{n}$. For each
straggler $i$, we denote its slowness $N_i$ by using the difference between its speed and
the average worker speed $\frac{S_\tau}{n}$. Assuming we have identified $m$
stragglers, we can represent $T_{bsp} = f(S_\tau, N, m)$.
Similarly, we can do the same for ASP and represent $T_{asp} = g(S_\tau, N, m)$.
\tian{We can use our own performance model for ASP and find a performance model for BSP.}
We will only switch from BSP to ASP if the training time saving $T_{\delta} = |
T_{bsp} - T_{asp}|$ is more than the switching overhead $T_{overhead}$.

It is easy to see that $\tau$ controls the upper bound in the number of
switches.
To account for prediction errors, e.g., underestimating the time required
when using the SGD that was switched to, we can extend the above idea by trying
to compensate the errors with conservative switching.



==> section/design_v2.tex <==
\section{Empirical and Theoretical Observations}

\section{\sysname Policy Design}
\label{sec:design}

\tian{Here is a new structure I am proposing: we can try to separate the empirical and theoretical explanations to a section called Empirical Observations and Theoretical Explanations before this section; and then in this section, we just describe the respective policies we have. Currently this section feels quite long and easily lost reviewers.} 

In this section, we propose the method of switching the synchronization based on different switching policies. We will go over several heuristics that can exploit the potentials of this approach, and some associated trade-offs and overheads to consider. We highlight several design choices we made for switching synchronization algorithms to optimize training performance on desired metrics. 

We focus on three main aspects in doing synchronization switch: 1) the basic heuristics that determine the ordering and number of switches needed in a training session. 2) the ideal timing for the actual switching point. 3) impact of important training hyper-parameters in different synchronization protocol and systematic ways to adjust them to ensure the performance of switching.

\subsection{The ordering of synchronization protocols}
\label{subsec:ordering}


The aim of our method is to achieve a test accuracy that is as high as when training exclusively with BSP, while still benefiting from (nearly) the same linear speedup in the per-epoch computation time afforded by ASP. %which is roughly linear in the number of workers.
%
Since we care only about minimizing the test error/maximizing test accuracy, our ultimate goal is to minimize the population loss--the loss value for the population distribution from which our dataset was sampled-- even if this does not lead to the lowest possible training loss value.
%
We argue here that using BSP in the earlier epochs and then switching to ASP can allow us to simultaneously accomplish both the goals of minimizing the population loss and improving the per-epoch computation time.

\eat{\tian{Is the argument regarding learning rate generalizable? Are we indicating that the common learning rate schedules often decay learning rate as the training goes on?}}
%
First, we note that the steps taken by momentum-SGD earlier in the training are much larger than those taken later in the training.  This is because, 1) at earlier epochs  the gradient tends to have a much larger magnitude, since it is further from a local minimum point  than at later epochs and 2) many state-of-the-art results use a decaying learning rate schedule, where the learning rate is much larger at earlier epochs than at later epochs.

Next, we argue (in \ref{sec_loss_landscape}) that at coarser scales corresponding to the large steps taken by the algorithm earlier in the training, the landscape of the population loss function resembles that of the training loss.
%
On the other hand, past empirical work \cite{kleinberg2018alternative, hochreiter1995simplifying, hochreiter1997flat, keskar2016large, smith2018bayesian, chaudhari2019entropy} suggests that at finer scales corresponding to the smaller steps taken later in the training, the landscape of the population loss is much smoother than that of the training loss. 
%


%
 Finally, we note that while stale gradients may be ineffective very early in the training when larger steps are taken by the algorithm, stale gradients can be used to effectively minimize the population loss later in the training, since the landscape of the population loss is much smoother on a finer scale corresponding to the smaller steps taken by the algorithm later in the training.
 This is because, at later epochs, the gradient of the population loss does not change as quickly each time the algorithm takes a step, which means that stale gradients  may still be able to provide useful information about the gradient of the population loss at the current point even though the stale gradients were computed at previous (but nearby) points.  This suggests that ASP can effectively minimize the training loss if it is used at later epochs.

On the other hand, at very early epochs, when the algorithm takes much larger steps, the gradient of the population loss may change very quickly at each step.  This means that stale gradients may not provide much information about the value of the gradient at the current point. This suggests using BSP early in the training, and then switching to ASP at a later epoch. This hypothesis is supported by our empirical results shown in Figure~\ref{fig:design_ordering}, which shows that using BSP at earlier epochs and switching to ASP at later epochs allows one to obtain a test error which is as low as in experiments using BSP during the entire training.

\begin{figure}[t!]
    \centering
    \includegraphics[width=\textwidth]{img/challenge_order.pdf}
    \caption{Converged accuracy of switching at 50\% of the the workload using different orders. Compared to the baseline BSP and ASP performance, switching from BSP to ASP can achieve the same level to that of BSP, while the reverse can only reach the level of ASP.}
    \label{fig:design_ordering}
\end{figure}

\begin{figure}[t!]
    \centering
    \begin{subfigure}[t]{0.2\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/cartoon_BSP.pdf}
        \caption{\textbf{BSP.}}
        \label{fig:cartoon_BSP}
    \end{subfigure}
    \,
    \,
    \,
    %
    \begin{subfigure}[t]{0.2\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/cartoon_ASP.pdf}
        \caption{\textbf{ASP.}}
        \label{fig:cartoon_ASP}
    \end{subfigure}
  %
        \begin{subfigure}[t]{0.2\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/cartoon_BSP_to_ASP.pdf}
        \caption{\textbf{Switching, BSP to ASP.}}
        \label{fig:cartoon_BSP_to_ASP}
    \end{subfigure}
    %
    \,
    \,
    \,
          \begin{subfigure}[t]{0.2\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/cartoon_ASP_to_BSP.pdf}
        \caption{\textbf{Switching, ASP to BSP.}}
        \label{fig:cartoon_ASP_to_BSP}
    \end{subfigure}
    %
    \caption{Illustrations of various combinations of BSP and ASP on a simple smooth loss function (blue level sets). All algorithms have larger step sizes in earlier epochs (due to larger learning rates and larger gradient magnitudes earlier in the training).  This means that, in earlier epochs, the gradient changes quickly at each step and stale gradients (red) are much less reliable than non-stale gradients (black).  Thus algorithms which use ASP earlier in the training may have a difficult time settling into a local minimum region where the gradient is small (b, d). This is true even if one switches from ASP to BSP (d) as the algorithm may get stuck in a saddle point once the learning rate has decayed, causing it to take a long time to escape the saddle point.  In contrast, if one only uses stale gradients at later epochs once the algorithm is closer to a minimum point, the stale gradients will be low-bias estimates for the true gradient and will still allow the algorithm to reach the minimum point (c).}
\end{figure}


\begin{figure}[t!]
    \centering
    \begin{subfigure}[t]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/Cartoon_training_loss_BSP.pdf}
        \caption{\textbf{BSP.}}
        \label{fig:cartoon_BSP_training_loss}
    \end{subfigure}
    \,
    \,
    \,
    %
    \begin{subfigure}[t]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/Cartoon_training_loss_BSP_ASP.pdf}
        \caption{\textbf{BSP to ASP.}}
        \label{fig:cartoon_ASP_training_loss}
    \end{subfigure}
    %
    \caption{The training loss (greed solind curve) is not as smooth as the population loss  (blue dashed curve).  Thus, the stale gradients used by our algorithm (b) do not allow it to find the minimum of the training loss as well as BSP (a).  However, it is still able to find the a point which minimizes the population loss as well as BSP.}
\end{figure}

\begin{remark}[Can switching from BSP to ASP also minimize the training loss?]
%
In the previous discussion we have used the fact that the population loss is oftentimes much smoother than the training loss.
%
For this reason, even if one only uses stale gradients later in the training when the algorithm takes smaller step sizes, the gradient of the training loss may still change rapidly at each step of the algorithm despite the fact that the gradient of the population loss may not be changing as quickly.
%
This suggests that, while using ASP later in the training may allow one to effectively minimize the population loss, it may still not allow one to minimize the training loss.
%
This is exactly what we observe in our experiments: while switching from ASP to BSP \shijian{BSP to ASP?} allows one to minimize the test error (and hence the population loss) as effectively as using BSP alone, the training loss remains much higher than in experiments where BSP alone is used.

\end{remark} 

We showed that doing BSP first then switching to ASP could effectively minimizing population loss, as well as to escape certain saddle points in gradient descent. It also illustrates the need to switch only once during the training, as switching multiple times would defy the advantages and characteristics we want to emphasize in each of the synchronization protocol while introducing more overhead and noise in the training due to framework limitation. We will talk about the noise of switching in Section~\ref{subsec:hyperparameter}, and quantify the overhead in Section~\ref{sec:eval}.

\paragraph{Population loss landscape at different scales}\label{sec_loss_landscape}
 There is much empirical and heuristic evidence that the  population loss is in fact much smoother than the training loss. 
%
 For instance, it has been observed that sharp local minima of the training loss -- minima where the training loss  is only low in a small region near the minimum point -- oftentimes do not correspond to a low test loss \cite{hochreiter1995simplifying, hochreiter1997flat, keskar2016large, smith2018bayesian, chaudhari2019entropy}.
%
On the other hand, 'flat' local minima of the training loss-- local minima where the training loss remains low in a wide region containing the local  minimum point-- in many cases also minimize the test loss.
%
Moreover, it has recently been shown that minimizing a 'smoothed' version
of the training loss can lead to a test error that is as low as, or oftentimes
even lower than, if one were to minimize the training loss itself. 
%
Here the smoothed loss function is the convolution of the loss function with
the distribution of the batch gradient noise (the variance of the noise depends
on the batch size) \cite{kleinberg2018alternative}.

This evidence suggests that the population loss is much smoother than the training loss, and is in fact closer to a 'smoothed' version of the training loss convolved with a the distribution of the batch gradient noise rather than the original training loss. This suggest that our population loss will have a landscape that is smooth at a finer scale on the order of the learning rate used later in the training.  On the other hand, at coarser scales--on the order of the large learning rate used earlier in the training--we expect the landscape of the population loss to be much closer to the training loss. In other words, earlier in the training, when a large step size is used, the change in the training loss and population loss at each step should be roughly the same, and the ratio of the change in the population loss to the change in training loss should be close to 1. Later in the training, when a much smaller learning rate is used, this ratio could be very far from 1.

\subsection{Switching policies}

In this subsection, we provide the sketch for our proposed switching policies, facing different both internal factors that are inherent to the deep learning and distributed training themselves, and external factors such as impact from stragglers or heterogeneous training environment. 

\paragraph{\textbf{Binary-search-based policy to find near-optimal switching point}}

Using the observations found in Section~\ref{subsec:ordering}, we have established basic heuristics in effectively doing synchronization switching: train with BSP first, then switch to ASP only once and train to convergence. The next logical step is to find when to do the switching. 

Assume a homogeneous and stable training environment, given a deep learning workload, there are hundreds of switching points if we treat each epoch as a potential switching point, or tens of thousand if we treat each step/mini-batch as one. We raise an hypothesis that since at a coarse-scale before convergence, the gradient descent curve is a monotonically non-increasing slope, the effect of switch timing on test accuracy is in reverse, a monotonically non-decreasing curve in positive correlation to the proportion of BSP training done in the total training workload. 

We conducted a group of empirical experiments to prove the hypothesis, training the ResNet32 on Cifar-10 dataset workload with an 8-worker cluster, using the detailed settings and hyper-parameters described in Section~\ref{sec:eval}, splitting the total workload with different ratios of BSP and ASP. We repeated each setting 5 times to reduce the inherent variance of distributed training performance, which is a technique commonly used in related research~\cite{goyal2017accurate}. We first chose 5 points: 0\% (which is in fact pure ASP), 25\%, 50\%, 75\% and 100\% (which is in fact pure BSP), then we divided the [0\%, 25\%] segment into finer segments with a 5\% increment, and an additional point at 2.5\%.

\begin{figure}[t!]
    \centering
    \includegraphics[width=\textwidth]{img/intuition_search.pdf}
    \caption{Converged accuracy vs. BSP proportion. The curve is as we hypothesized monotonically non-decreasing within a certain margin of error.}
    \label{fig:search_empirical}
\end{figure}

As observed in~\ref{fig:search_empirical}, the converged accuracy using synchronization switching at different workload split is monotonically non-decreasing within a margin of error of 0.01. Given that BSP is strictly slower in terms of training throughput compared to ASP, it means that the less BSP proportion is in the mixed synchronization training, the faster it is able to complete the given training workload. This finding enables a simple binary-search-based policy to find a near-optimal switching point for a given workload. \shijian{Might need to phrase better}Assume that the workload isn't an one-off training job, which means that it will see repeated training, either for fine tuning, or using the model on a different dataset for a similar task. This workload can either be seen before or unseen. Formally, we formulate the searching process as an optimization problem:

\begin{equation*}
\begin{aligned}
& \underset{s}{\text{minimize}}
& & T(s) \\
& \text{subject to}
& & \alpha(s) \geq \alpha(s_{max}), \\
&&& s_{min} \leq s \leq s_{max}
\end{aligned}
\end{equation*}

Where $s$ denotes the switching point during training, $T$ the total training time to complete the given workload, and $\alpha$ the converged accuracy using the current switching point $s$. $s_{min}$ and $s_{max}$ are ASP and BSP, respectively.

\begin{algorithm}
\caption{Searching algorithm for near-optimal switching point}
\begin{algorithmic}
\STATE \textbf{Inputs:} Threshold $\beta$, Search attempt limits $N_{limit}$, Target accuracy $\alpha$, Runs to train for each setting $N_{run_{limit}}$
\IF{Target accuracy not provided}
\STATE Train the model with BSP $N_{run}$ times to get converged accuracy $\alpha_1 ... \alpha_{N_{run_{limit}}}$, and set $\alpha = \frac{1}{N_{run_{limit}}}\sum_{i=1}^{N_{run_{limit}}}\alpha_i$
\ENDIF
\STATE $UPPER = 100, LOWER = 0, N_{attempt}$
\WHILE{$N_{attempt} < N_{limit}$}
\STATE $Timing = \frac{(UPPER + LOWER)}{2}$
\STATE $N_i = 0$
\WHILE{$N_i < N_{run_limit}$}
\STATE Train $Timing\%$ of workload using BSP
\STATE Train $1 - Timing\%$ of workload using ASP to get converged accuracy $\alpha_i$
\STATE $i = i + 1$
\ENDWHILE
\STATE $\alpha_{N_{attempt}} = \frac{1}{N_{run_{limit}}}\sum_{i=1}^{N_{run_{limit}}}\alpha_i$
\IF{$\alpha_{N_{attempt}} >= \alpha - \beta$}
\STATE $UPPER = Timing$
\ELSE
\STATE $LOWER = Timing$
\ENDIF
\ENDWHILE
\label{alg:binary}
\end{algorithmic}
\end{algorithm}

In Algorithm~\ref{alg:binary}, we specify a limit for number of settings $N_{limit}$ we want to explore, since from the observation in our empirical experiment, the speedup provided for switching earlier over a small percentage of workload is negligible. $\beta$ is the margin of error for converged accuracy due to the stochastic nature of deep learning and distributed training, and should either be specified by the user or set automatically (see~\ref{sec:eval} for details). To further reduce variance, we set the number of runs for each switch point $N_{run_{limit}}$. A large $N_{run_{limit}}$ can reduce sub-optimal results, but increase the search cost. In reverse, a small $N_{run_{limit}}$ can reduce search cost, but increase the possibility of sub-optimal results. $\alpha$ is the target converged accuracy in the constraints. 

\paragraph{\textbf{Straggler-based switching policies}}

In this subsection, we propose policies that could alleviate training throughput degradation in a heterogeneous or unstable environment. Due to the inherent advantage of ASP to provide resilience to distributed training, the synchronization switching should be able to capitalize this property and provide similar level of resilience in the training session as well, while still be able to achieve BSP level of converged accuracy. 

One important aspect to the problem we want to solve here is the assumption that the slowness will not be permanent on the workers, but occurs randomly. Additionally, slowness in the cluster doesn't apply to the majority of workers. In the case of a cluster with many permanent stragglers, it would lead to sub-optimal performance to conduct distributed training no matter what synchronization protocol is used, even with a pure ASP setting. 

Assuming a training environment that has random slowness in the workers due to bad network connection, limited bandwidth, or resource contention, which is common in the commodity public clouds, we want to minimize the impact of the slowness imposed on training throughput. To achieve this goal, we avoid overlapping BSP session of training and the occurrence of slowness. 
 
An intuitive policy is to start with the basic heuristics found in subsection~\ref{subsec:ordering}, where we first apply BSP in training. Under this circumstance we either know the optimal switching point or is in the process of searching for one, which means we have a designated BSP workload proportion $P_{BSP}$. For a given training workload and cluster of $n$ servers, assume the average training speed for a worker in the cluster is $S_\tau$ and standard deviation is $C_\tau$ between $[0, \tau]$, a worker is marked as a straggler if its speed falls outside $\frac{S_\tau}{n} \pm \frac{C_\tau}{n}$. For each straggler $i$, we denote its slowness $N_i$ by using the difference between its speed and the average worker speed $\frac{S_\tau}{n}$. Assuming we have identified at least 1 straggler in the cluster, we switch to ASP if it's currently using BSP. We switch back from ASP to BSP once the slowness of the straggler(s) is gone, and finish the designated BSP proportion $P_{BSP}$. This process can happen more than once in case straggler slowness is a recurrent event. This policy works fine when the period of slowness is short and infrequent. But facing long and frequent slowness in the cluster, this policy could lead to the situation where the total amount of BSP training is smaller than $P_{BSP}$, or the BSP is applied in a later stage of training, going against our findings in subsection~\ref{subsec:ordering} and leading to sub-optimal converged accuracy for the trained model.

To combat this long and frequent occurrence of slowness, we propose an alternative elastic-training-based policy. Assuming the same environment and training cluster setup as described above, in this policy, we still train with BSP first by default. When we detected $m$ stragglers in a training cluster of size $n$, we shrink temporarily the cluster size to be $n - m$, excluding the stragglers, to finish the designated BSP proportion $P_{BSP}$. Once $P_{BSP}$ is reached, we switch to ASP with all $n$ workers no matter if some of them are experiencing slowdown. In this policy we can adhere to the heuristics found in subsection~\ref{subsec:ordering}, preserving both the switching order and times. Since BSP speedup usually is sub-linear, a short period of using fewer workers will not likely negate the throughput gain from the linear speedup of ASP training. And more importantly, the converged accuracy could still be guaranteed to be on the same level that was intended to be.

\paragraph{\textbf{Dynamic switching policy}}

\shijian{Tian had an idea of briefly mentioning the idea here, and put more details into appendix, like what the Tiresia paper did.}

\subsection{Hyper-parameters adjustments}
\label{subsec:hyperparameter}

In this subsection, we discuss several key hyper-parameters of a typical training session, their impact on the training performance, both ASP and BSP, and some necessary changes we made to accommodate the switching of synchronization protocols.

Since our work isn't about hyper-parameter tuning, we are not focusing on finding the optimal set of hyper-parameters for a specific training setting. When given the workload and a cluster with size $n$ for training, we take in an initial set of hyper-parameters as input values provided by the end user. Namely, we expect mini-batch size $B$ and learning rate $\eta$ to be specified as the basis for our adjustment. We aim to automatically change the value of these hyper-parameter according to the synchronization protocol used, and requires no manual tuning and optimization, in order to ensure the performance of the synchronization switching on the desired key metrics.

\paragraph{Mini-batch size.} The difference in the logic of the training workflow and the implementation of different synchronization protocols in the deep learning framework we are using, BSP and ASP have different views on the notion of batch size. In BSP training, the batch size is global, seen as an aggregated value to be distributed on the workers. However, in ASP training the batch size is treated as a local value specific to each worker. This means that the effective batch size for BSP $B_{BSP}$ is $B_{ASP} * n$, where $B_{ASP} = B$ is the effective batch size in ASP training, and $n$ the cluster size. This aligns with the findings of previous studies~\cite{goyal2017accurate}, where they observed that the BSP training batch size should scale with the cluster size.

\paragraph{Learning rate.} In previous studies it is observed that when the batch size is scaled in the training session, the learning rate $\eta$ should also scale accordingly. For BSP training, scaling $\eta_{BSP}$ linearly to batch size $B_{BSP}$ is proven to be effective in ensuring good convergence on the model~\cite{goyal2017accurate}. We applied the same \textit{linear scaling rule} on BSP training, and set $\eta_{BSP} = n * \eta$, where $\eta$ is the base learning rate, and $n$ the cluster size. 

Similarly, we scale the learning rate for ASP training as well. Contrary to BSP, the batch size doesn't increase from the perspective of the training session. Thus we don't scale up the learning rate. However, as the cluster size increases, more stale and noisy gradients from different workers are introduced into the training session. These gradients can point to different directions in the gradient descent slope, and with a large enough learning rate, can cause the model to diverge resulting in failed training. In our empirical experiments, we have found that the base learning rate can cause divergence in training. Thus we scale down the learning rate for ASP $\eta_{ASP}$ in proportion to $n$. We found a sub-linear scaling factor of $\frac{1}{\sqrt{n}}$ to be more effective than the linear scaling factor of $\frac{1}{n}$, which caused $\eta_{ASP}$ to be too small and led to slower and worse convergence due to potentially being trapped in saddle points.

\shijian{I was going to include the adjustment to learning rate decay schedule here as well. However, I feel like it is not really a design choice - but rather an implementation detail that we HAVE to do to ensure the correctness of training with ASP and BSP. If we didn't do it then the learning rate decays at different epochs into training, diverging from the intended decay point. This discrepancy comes from the training loop being viewed from the view of steps instead of epochs. }

\paragraph{Momentum} Momentum is a popular technique in SGD that improves the convergence rate~\cite{rumelhart1986learning}. It helps accelerate SGD in the relevant direction and dampens oscillations of the gradients. Previous studies~\cite{lin2019dynamic} have found that in situations where the batch size changes, there might be negative impact on the training loss, and adjusting the momentum could alleviate the problem. Our empirical experiment shown in Figure~\ref{fig:sync_teaser_results:loss} confirms with this observation. However, we also found that while adjusting momentum could mitigate the spike in training loss, it also leads to lowered converged test accuracy. In our experiments we found that the spike in training loss doesn't impact the eventual converged test accuracy. Thus we leave the momentum unchanged.

==> section/design_v3.tex <==
% \section{Empirical and Theoretical Observations}

% % make sure to link this section and the next section about policies 

% \subsection{Which synchronization to use: BSP or ASP?}

% \input{latex-figs/exp_bsp_vs_asp}

% In this section, we look at the training throughput difference between using BSP and ASP with and without stragglers with the goal to identify suitable training scenarios.   

% \para{Observation One.} Training synchronously with BSP has slower throughput than training fully asynchronously with ASP. The throughput difference is exacerbated when stragglers are present in the training cluster. Figure~\ref{fig:exp_bsp_vs_asp} compares the respective training performance under different setups. 


% \subsection{Can we benefit from both BSP and ASP?}

% \input{latex-figs/sync_protocol_teaser_results}

% \input{latex-figs/exp_bsp_order_percentage}

% Given the respective pros and cons of BSP and ASP, we next investigate the feasibility of simultaneously achieving high-quality training with near-linear speedup. 
% % mention the result group in intro 

% \para{Observation Two.} It is not necessary to train with BSP for the entire workload to benefit from the high-quality converge accuracy. 



% % switching from BSP to ASP is better 



% % doing more BSP does not necessarily lead to higher accuracy. 

% We conducted a group of empirical experiments to prove the hypothesis, training the ResNet32 on Cifar-10 dataset workload with an 8-worker cluster, using the detailed settings and hyper-parameters described in Section~\ref{sec:eval}, splitting the total workload with different ratios of BSP and ASP. We repeated each setting 5 times to reduce the inherent variance of distributed training performance, which is a technique commonly used in related research~\cite{goyal2017accurate}. We first chose 5 points: 0\% (which is in fact pure ASP), 25\%, 50\%, 75\% and 100\% (which is in fact pure BSP), then we divided the [0\%, 25\%] segment into finer segments with a 5\% increment, and an additional point at 2.5\%.

% As observed in~\ref{fig:bsp_percentage}, the converged accuracy using synchronization switching at different workload split is monotonically non-decreasing within a margin of error of 0.01. Given that BSP is strictly slower in terms of training throughput compared to ASP \Lijie{We need to argue that BSP is still slower than ASP when there are no stragglers}, it means that the less BSP proportion is in the mixed synchronization training, the faster it is able to complete the given training workload. This finding enables a simple binary-search-based policy \Lijie{This policy seems that we do not have any insights and then choose a general way. How about considering the benefit of the loss descend range and the training time, e.g., the insight is to choose a switching point where the loss begins to decrease slow (the slope is going to be flat). We can define a benefit and try to optimize this benefit} to find a near-optimal switching point for a given workload. 

% \subsection{Do we need to adjust the configuration after switching?}

% % the potential problem if we don't switch configuration 






\section{\sysname Policy Design}
\label{sec:design}

In this section, we introduce a set of policies that determine \emph{how and when to switch to a different synchronization}. This includes offline policies that target recurring jobs (Sections~\ref{subsec:ordering} and \ref{subsec:offline_binary_search}), online policies that react to training status (Section~\ref{subsubsec:online_policies}), and policies for adjusting hyper-parameters.  

% \tian{needs to be rewritten. will do later}
% In this section, we propose the method of switching the synchronization based on different switching policies. We will go over several heuristics that can exploit the potentials of this approach, and some associated trade-offs and overheads to consider. We highlight several design choices we made for switching synchronization algorithms to optimize training performance on desired metrics. 

% We focus on three main aspects in doing synchronization switch: 1) the basic heuristics that determine the ordering and number of switches needed in a training session. 2) the ideal timing for the actual switching point. 3) impact of important training hyper-parameters in different synchronization protocol and systematic ways to adjust them to ensure the performance of switching.

\subsection{Protocol Policy: Which to Use and in What Order?}
\label{subsec:ordering}

% the readers should be clear that 
% 1. choosing between asp and bsp makes more sense than selecting from a set of synchronization protocol 
% 2. why it makes sense to use BSP first. 

In this work, we focus on selecting between two synchronization protocols, i.e., fully synchronous (BSP) and fully asynchronous (ASP). As described previously in Section~\ref{sec:intro}, there are a plethora of other protocols that provide different trade-offs between training throughput and converged accuracy. Mixing in these in-between training protocols might produce a slightly better outcome due to larger decision spaces; however, these in-between protocols can be complicated to use due to lack of framework support and the use of extra hyper-parameters~\cite{dutta2020slow,jiang2019novel,hsieh2017gaia}.
% , but also unnecessarily increases the complexity \Oren{This sentence is a bit vague.  I would say something like ``However, these ``in-between" training protocols can be very complicated to implement in practice on different architectures"  (is what I wrote here correct? If not, then what are the disadvantages of the other ``in-between
% protocols?  I think we need to be a bit more specific here about the disadvantages of the other protocols).}. We leave the exploration of selecting the best protocol from a set of protocols as part of future work \Oren{Maybe we should remove this sentence, if the point is that the available training protocols are too complicated to implement in practice}. 

Our first policy states that we should start the training with BSP and then switch to ASP when the following conditions are satisfied: 
\1 When switching to ASP yields a similar converged {\em test} accuracy (but perhaps a lower {\em training} accuracy) as continuing with BSP;
% \1 when continuing with BSP will yield similar converged accuracy to with ASP \Oren{I would replace this sentence with ``When switching to ASP yields a similar converged {\em test} accuracy (but perhaps a lower {\em training} accuracy) as continuing with BSP"} 
\2 when transient stragglers arise in the training cluster. We will describe the policies that verify both conditions to determine the switching timing in Section~\ref{subsec:timing_policy}. 

%%
\input{latex-figs/exp_bsp_order_percentage}
%%

% \para{Empirical Evidence.} 
\subsubsection{Empirical Analysis}
To evaluate our hypothesis that running BSP at earlier epochs and switching to ASP at later epochs allows one to obtain a test error which is as low as using BSP during the entire training, we conducted two experiments. The experiments train the ResNet32 model on the CIFAR-10 dataset with an 8-worker cluster, with each configuration repeated five times (additional experiment details can be found in Section~\ref{subsec:eval_methodology}).
%
First, we evaluate the converged accuracy when training with different combinations of BSP and ASP protocols, as shown in Figure~\ref{fig:bsp_order}. We observe that training with BSP for 50\% of the workload and then switching to ASP outperformed its counterpart, i.e., ASP $\rightarrow$ BSP. Second, we examine the relationship between converged accuracy and the percentage of BSP training and find that training more with BSP does not necessarily lead to higher converged accuracy. As shown in Figure~\ref{fig:bsp_percentage}, the converged accuracy first increases with the percentage of BSP training and then stays on par with training entirely with BSP (i.e., 100\%). This observation also provides the basis for deriving the timing policy as described in Section~\ref{subsec:timing_policy}.

\subsubsection{Theoretical Explanations}
% \para{Theoretical Explanations.} 
Next we explain why using BSP in the earlier epochs and then switching to ASP can allow us to simultaneously accomplish both our goals of minimizing the \emph{population loss} (that is, the expected value of the testing loss) as effectively as when using \emph{static BSP}, and improving the per-epoch computation time.
%
Here, by static BSP (respectively, ASP), we mean the protocol where one uses only BSP (respectively, ASP) from start to finish.

First, we note that the steps taken by SGD earlier in the training are much larger than those taken later in the training.  This is because, \1 at earlier epochs  the gradient tends to have a much larger magnitude, and \2 we use a decaying learning rate schedule, where the learning rate is much larger at earlier epochs than at later epochs, a common practice when training deep learning models \cite{he2016deep, huang2017densely}.

% \tian{is it possible to provide argument without Appendix? Citation to prior work or simply citation to our own arXiv?}
% \Oren{I point to the ArXiv version for the remarks.  (I put the remarks in the appendix for now to save space, but they will only appear in the ArXiv version in the end).}
%
Second, we note that at coarser scales corresponding to the large steps taken by the algorithm earlier in the training, the landscape of the {\em population} loss  resembles that of the training loss (see Remark~\ref{rem_population_loss} in the extended version for more details~\cite{syncswitch-extended}).
%
% \shijian{6 citations here, we could reduce the amount by 2-4 in my opinion, consult Oren on which ones to cut. Also 5 of the same citations are grouped in the appendix already.} \Oren{I reduced the citations.} 
On the other hand, past empirical work~\cite{kleinberg2018alternative, hochreiter1995simplifying, keskar2016large} %\cite{hochreiter1997flat smith2018bayesian, chaudhari2019entropy}  
suggests that at finer scales corresponding to the smaller steps taken later in the training, the landscape of the population loss is much smoother than that of the training loss. 
%


%
 These two facts imply that while stale gradients may be ineffective very early in the training when larger steps are taken by the algorithm, stale gradients can be used to effectively minimize the population loss later in the training, since the landscape of the population loss is much smoother on a finer scale corresponding to the smaller steps taken by the algorithm later in the training (Figure \ref{fig:cartoon_training_loss}).
 %
 This is because, at later epochs, the gradient of the population loss does not change as quickly each time the algorithm takes a step, which means that stale gradients  may still be able to provide useful information about the gradient of the population loss at the current point even though the stale gradients were computed at previous (but nearby) points.  This suggests that using ASP at later epochs (Figure \ref{fig:cartoon_BSP_ASP_training_loss}) can allow one to minimize the {\em population} loss (and hence the testing loss) as effectively as static BSP (Figure \ref{fig:cartoon_BSP_training_loss}), despite the fact that static BSP can achieve a lower {\em training} loss value (see Remark \ref{rem_can_BSP_to_ASP_minimize_training_loss} in our extended version for more details~\cite{syncswitch-extended}).
 %
 
On the other hand, at very early epochs, when the algorithm is very far from a minimum point, the gradient of the loss function may have a very large magnitude and may change very quickly at each step \footnote{For instance, consider the simple 4'th-order polynomial $f(x) = x^4$.  For this function, the gradient $f'(x) = x^3$ changes more quickly when $x$ is further from the minimum point $x=0$.  Roughly speaking, for loss functions defined by deep neural networks there can be many (multivariate) high-order terms, with the order of the terms growing with the depth of the network.} 
%
Thus, in protocol policies where ASP is used early in the training, its stale gradients may not provide much information about the value of the gradient at the current point, and may cause ASP to exhibit unstable behavior early in the training (Figures \ref{fig:cartoon_ASP} and \ref{fig:cartoon_ASP_to_BSP}), preventing ASP from effectively decreasing the loss value. 
%
To avoid this unstable behavior, one should use BSP in the very early stages of the training, and only switch to ASP at a later epoch once the learning rate is lower and the gradients are changing more slowly (Figure \ref{fig:cartoon_BSP_to_ASP})
%
(See Remark \ref{rem_why_not_ASP_to_BSP} in our extended version for additional discussions~\cite{syncswitch-extended}.)




% \Lijie{I just list the key questions and solution insights according to my understanding. It maybe not  correct, but using question-answer style is clearer and interesting. We can adjust the respective descriptions later.}

% \Lijie{We first state our goals and polices, then argue why we choose this policy, i.e., how we solve the sub-questions. Note that we need to clarify the definition of convergence rate, loss, throughput, accuracy. Test accuracy and population loss may be hard to understand for non-ML experts.}

% \Lijie{add begin}
% Our goal is to let the model converge as fast as possible, i.e., achieve high training throughput as well as high accuracy (comparable with the pure BSP, measured by test accuracy). Since BSP suffers from low training throughput and ASP suffers from low accuracy, we can perform two switching polices to balance them: changing BSP to ASP, or changing ASP to BSP when suffering from throughput/accuracy problem.

% Our selected policy: Use BSP first and then change it to ASP when necessary until the end.

% Why using this policies, there are three sub-questions.

% (1) Why using BSP first instead of ASP? We select BSP as the initial protocol because we care more about the convergence rate (loss curve) in the first n stages (epochs/steps). The advantage of using BSP first is that it can make the loss drops down at the right direction. This is important for the first n stages , because the loss varies a lot (in a large range) in the first n stages. If the direction is correct in the first n stages, the loss will drops very fast. The learning rate is usually very large at the first n stages (e.g., 10 times of that in the following n stages), which leads to large gradient/parameter increments. if using ASP in the first n stages, the large gradient/parameter variation will make the loss curve go to a wrong direction with a large distance, leading to more steps to return to normal.  

% (2) Why changing BSP to ASP can improve the throughput while maintaining the accuracy (achieving comparable accuracy?) Changing BSP to ASP can improve the throughput, which has been discussed in Background. The only question is if it can maintain the accuracy.
% At later stages, the parameter increments is very small (learning rate is very small). Training model is to look for the optimum parameters in a small range. At this time, the searching efficiency is more important. ASP is faster , even at wrong direction, it is still within the sub-optimum range and and  search a relatively larger sub-optimum range.
% Give some evidences and comparison by BSP to ASP and ASP to BSP.

% (3) Why switching only once? i.e, why not change ASP to BSP again?
% At later stages, changing BSP to ASP is unnecessary. The reason is that the parameter increment is very small, The increments of ASP and BSP are very similar.
% \Lijie{add end}


\input{latex-figs/illustration_bsp_vs_bsp2asp}

\input{latex-figs/illustration_switching_order}



% \begin{remark}[Why not do multiple switches?]
% %
% In our current policy, we use BSP in the earliest epochs of the training and then switch to ASP for the remaining epochs.
% %
% However, one may also consider policies where one switches multiple times between the BSP and ASP protocols, before permanently switching to ASP for the remaining epochs.
% %
% In theory, performing multiple switches early in the training may sometimes allow for an even greater speedup.
% %
% However, in practice we have found that performing multiple switches introduces significant overhead costs which greatly out-ways the benefits of switching multiple times early in the training.
% %
% This is especially true since, in practice, we have found that, even with only one switch from BSP to ASP, one only needs to use BSP in roughly the first 5\%-10\% of the epochs (see Section \ref{subsec:perf_search_based_policy} for details of empirical results).
% %
% Further reducing the time spent on BSP by performing multiple switches early in the training would only marginally decrease the average per-epoch runtime, at the cost of a much greater overhead due the increased number of switches.
% %
% \end{remark}

%In summary, we have argued that performing BSP first then switching to ASP can effectively minimize the population loss (and hence the test loss), by allowing SGD to train in a stable manner early in the training via BSP while allowing for an increased throughput via ASP at later epochs. 
% tian: talk about why only switching one time in the evaluation section

% Moreover, in practice we have found that there is no advantage to switching more than once during the training, as it would introduce a large overhead and noise to the training due to framework limitations while only offering a small improvement in the average per-epoch runtime.






\subsection{Timing Policy: When to Switch?} 
\label{subsec:timing_policy}

% connection with the previous subsections 
% how we decide the timing under different conditions 
% why they are effective 
% and potentially experiments to show that they are effective 

Next, we introduce \sysname's timing policy which determines when to switch between BSP and ASP. Deciding the proper timing to switch is an important problem as it not only impacts the converged accuracy but also the training time. Furthermore, it is a challenging problem as both model-specific factors such as training progress and runtime factors such as slow nodes can impact the timing. Specifically, we develop both offline and online policies that are suitable to use under different training conditions. 

\subsubsection{Offline Policy via Binary Search}
\label{subsec:offline_binary_search}

% \input{latex-algos/algo_binary_search}

% \shijian{Some modifications here: added missing explanation of notations, the formulation is also changed. For the function I think just T(s) would be correct because otherwise not searching would be the best solution because no addition training sessions were done. Also changed minimize to arg min, because we are trying to use the offline policy to find the switching point, which should be $s$ and not the total time.}
Based on our empirical observation that BSP is strictly slower than ASP, with or without stragglers, and that the converge accuracy increases monotonically with the amount of BSP training, we formulate the searching process as a binary search problem.
% as an optimization problem. 
%
Specifically, for a given training workload, our goal is to find a switching point $s$ that yields a converged accuracy $\alpha(s)$ that satisfies $\alpha(s_{min}) \leq \alpha(s) \pm \alpha_{threshold} \leq \alpha(s_{max})$, where $s_{min}$ and $s_{max}$ represents training with ASP and BSP, respectively.
Further, the corresponding training time $T(s)$ should be as close to $T(s_{min})$ as possible, i.e., switching as early from BSP to ASP as possible. Lastly, we want to find $s$ in as fewer trial training sessions as possible to reduce search overhead. 
%
% Tian: commented out the following, because it is actually quite difficult to talk about the optimization 
% \begin{equation*}
% \begin{aligned}
% % & \underset{s}{\text{arg min}}
% & \argmin_{s}
% & & T(s) \\
% %+ \sum\limits_{i=0}^{N(s)} T(i), \\
% % & \text{subject to}
% & \st
% & & \alpha(s_{min}) \leq \alpha(s) \pm \alpha_{threshold} \leq \alpha(s_{max}), \\
% &&& s_{min} \leq s \leq s_{max}.
% \end{aligned}
% \end{equation*}

% Where $s$ and $T(s)$ denote the switching point and the total training time to complete the given workload, respectively. $N(s)$ is the number of times we need to search to find the switching point. $\alpha$ represents the converged accuracy, while $\alpha_{threshold}$ is the margin of error for stopping at the solution switching point, which in our experiments was set to 0.001; $s_{min}$ and $s_{max}$ are ASP and BSP, respectively. As $s$ represents a continuous variable, we chose to parameterize it at a logical time unit of per mini-batch. 
%
The pseudo-code for our binary search algorithm can be found in our extended technical report~\cite{syncswitch-extended}. 
% Appendix~\ref{appendix:sec:pseudo} \tian{technical report or arXiv?}.
%
% In Algorithm~\ref{alg:binary}, we specify a limit for number of settings $N_{limit}$ we want to explore, since from the observation in our empirical experiment, the speedup provided for switching earlier over a small percentage of workload is negligible. $\beta$ is the margin of error for converged accuracy due to the stochastic nature of deep learning and distributed training, and should either be specified by the user or set automatically (see~\ref{sec:eval} for details). To further reduce variance, we set the number of runs for each switch point $N_{run_{limit}}$. A large $N_{run_{limit}}$ can reduce sub-optimal results, but increase the search cost. In reverse, a small $N_{run_{limit}}$ can reduce search cost, but increase the possibility of sub-optimal results. $\alpha$ is the target converged accuracy in the constraints. 
%
In summary, for each distributed training workload, we can use a binary search algorithm to find the best switching point $s$ at which point \sysname will switch from training with BSP to ASP. We analyze the cost and performance tradeoff in Section~\ref{subsec:search_overhead}.

\subsubsection{Online Policies for Handling Stragglers}
\label{subsubsec:online_policies}

The offline policy described above provides us a good basis for speeding up distributed training while achieving high-quality test accuracy. However, it does not account for runtime factors including stragglers and also requires upfront search cost. In this section, we introduce two types of policies that are designed to react to the training status. 

% 1. transient stragglers do not often impact time, but can impact accuracy in \sysname? § empirical observation 

We target transient stragglers, e.g., nodes that exhibit temporary slowdown due to datacenter network or server resource contention, a non-rare occurrence when using public cloud~\cite{duan2017cloud,Li2010-dm}. 
%
Note that permanent stragglers are best dealt with by requesting replacement~\cite{Or2020-nh,Peng2018-mw}---simply switching to a more straggler-tolerant protocol like ASP might mitigate but not eradicate the performance impact. 
%
More explicitly, we consider the policies that deal with permanent stragglers as complementary work and therefore skip the discussion and evaluation of such policies. 
%
For ease of exposition, we assume that each occurrence of the slowness lasts at most the time to provision a new cloud server---we use 100 seconds based on empirical measurement reported by prior work~\cite{Li2020-bk}.
% \footnote{If the slowness duration of a server is constantly higher than the time to acquire a new one, it will be more effective to provision a new one.}. 
We further assume that \1 each node can become a straggler at any time during the training; \2 the number of unique straggler nodes is less than the cluster size.  
% these stragglers can appear randomly during the training 
Our goal is to design policies that adequately deal with the potential impact on the training time which also work \emph{in tandem} with the other policies of \sysname described above. 

We introduce two policies, both centering on the key insight that any transient straggler-oriented policies only need to react before the switch timing for a given workload. This is because once a training session is switched to ASP, we consider it immune from the impact of transient stragglers. 
% 
The first \emph{greedy} policy simply switches to ASP (if it is not already using ASP, which can happen if two stragglers overlap) when a straggler is detected; once the cluster is free of any stragglers and the aggregate BSP training has not been satisfied, it will switch back to training with BSP. This policy therefore might result in multiple synchronization switches, which overhead as we will show in Section~\ref{subsec:practical_overhead} can be in the order of tens seconds. 

To circumvent the switching overhead, we design an elastic-based policy that removes any detected stragglers from the current cluster so as to complete the specified amount of BSP training free of stragglers. Once the designated BSP workload is fulfilled, it will then restore the cluster size and train the remaining workload with ASP. As such, this elastic-based policy is more resistant to the frequency of straggler occurrences.
% 
For both policies, we leverage the historical average training throughput to detect the stragglers, a common technique used in various application domains~\cite{Li2020-bk, xie2010improving}. 
%
Specifically, a worker $k$ is identified as a straggler if its training throughput over a sliding window $S_k$ is lower than the difference between the cluster average and standard deviation $S-\sigma$, for a number of consecutive detection windows. 

% In this subsection, we propose policies that could alleviate training throughput degradation in a heterogeneous or unstable environment. Due to the inherent advantage of ASP to provide resilience to distributed training, the synchronization switching should be able to capitalize this property and provide similar level of resilience in the training session as well, while still be able to achieve BSP level of converged accuracy. 

% One important aspect to the problem we want to solve here is the assumption that the slowness will not be permanent on the workers, but occurs randomly. Additionally, slowness in the cluster doesn't apply to the majority of workers. In the case of a cluster with many permanent stragglers, it would lead to sub-optimal performance to conduct distributed training no matter what synchronization protocol is used, even with a pure ASP setting. 

% Assuming a training environment that has random slowness in the workers due to bad network connection, limited bandwidth, or resource contention, which is common in the commodity public clouds, we want to minimize the impact of the slowness imposed on training throughput. To achieve this goal, we avoid overlapping BSP session of training and the occurrence of slowness. 
 
% \Lijie{Our policy: using one sentence to summarize our policy. e.g., We switch the BSP to ASP when the stragglers last for a XX time according to the average speed?}

% An intuitive policy is to start with the basic heuristics found in subsection~\ref{subsec:ordering}, where we first apply BSP in training. Under this circumstance we either know the optimal switching point or is in the process of searching for one, which means we have a designated BSP workload proportion $P_{BSP}$. For a given training workload and cluster of $n$ servers, assume the average training speed for a worker in the cluster is $S_\tau$ and standard deviation is $C_\tau$ between $[0, \tau]$, a worker is marked as a straggler if its speed falls outside $\frac{S_\tau}{n} \pm \frac{C_\tau}{n}$. For each straggler $i$, we denote its slowness $N_i$ by using the difference between its speed and the average worker speed $\frac{S_\tau}{n}$. Assuming we have identified at least 1 straggler in the cluster, we switch to ASP if it's currently using BSP. We switch back from ASP to BSP once the slowness of the straggler(s) is gone \Lijie{In the previous section, we aruge that we only switch once once}, and finish the designated BSP proportion $P_{BSP}$. This process can happen more than once in case straggler slowness is a recurrent event. This policy works fine when the period of slowness is short and infrequent. But facing long and frequent slowness in the cluster, this policy could lead to the situation where the total amount of BSP training is smaller than $P_{BSP}$, or the BSP is applied in a later stage of training, going against our findings in subsection~\ref{subsec:ordering} and leading to sub-optimal converged accuracy for the trained model.

% To combat this long and frequent occurrence of slowness, we propose an alternative elastic-training-based policy. Assuming the same environment and training cluster setup as described above, in this policy, we still train with BSP first by default. When we detected $m$ stragglers in a training cluster of size $n$, we shrink temporarily the cluster size to be $n - m$, excluding the stragglers, to finish the designated BSP proportion $P_{BSP}$. Once $P_{BSP}$ is reached, we switch to ASP with all $n$ workers no matter if some of them are experiencing slowdown. In this policy we can adhere to the heuristics found in subsection~\ref{subsec:ordering}, preserving both the switching order and times. Since BSP speedup usually is sub-linear, a short period of using fewer workers will not likely negate the throughput gain from the linear speedup of ASP training. And more importantly, the converged accuracy could still be guaranteed to be on the same level that was intended to be.



% \para{Based on Training Status.} 
% Additionally, we can also dynamically determine the switch timing from BSP to ASP based on training status (see Appendix~\ref{sec:dynamic_switching}).
% % Next we give a criterion for dynamically determining the switching time from BSP to ASP based on training status.
% %
% However, we have found that, in practice, implementing dynamic switching criteria  requires extensive modifications to the existing frameworks and would lead to significant measurement overhead.
% %
% For this reason, we do not include a switching criterion based on training status in our code and experiments.




\subsection{Configuration Policy: How to Adjust Hyper-parameters?}
\label{subsec:hyperparameter}

\input{latex-figs/exp_hyperparameters}

% why we need to adjust hyperparameter after switching. 
Hyper-parameters are commonly considered important for training performance~\cite{senior2013empirical, smith2017don}. In our work, we also observe non-negligible differences with different hyper-parameters \emph{after switching} from BSP to ASP.
For example, in Figure~\ref{fig:batch_size_scaling}, we show that the difference in training throughput can be up to 2X with different batch sizes; in Figure~\ref{fig:momentum_scaling}, we observe up to 5\% converged accuracy differences using different momentum scaling techniques. 
As such, it is important to choose suitable hyper-parameters after synchronization switching so as to retain the training benefits. 

% how we set the hyperparameters
Through empirical investigations, we find that adjusting the following three hyper-parameters: \emph{mini-batch size}, \emph{learning rate}, and \emph{momentum} sufficient. 
Note, since our work is not about hyper-parameter tuning, we do not focus on finding the optimal hyper-parameters set for a specific training setting; rather, we are aiming to automatically change the value of these hyper-parameters based on the synchronization protocol in use. 
We assume the deep learning practitioners will provide an initial set of hyper-parameters, e.g., a mini-batch size of $B$ and a learning rate of $\eta$, given the training workload and a GPU cluster of $n$ nodes. 

To start the training with BSP, we will configure the mini-batch to be $nB$. This configuration is based on both the implementation of BSP batch size in the TensorFlow framework (i.e., as a global value distributed to each worker) and prior work's suggestion of setting BSP batch size proportionally to the cluster size~\cite{goyal2017accurate}. Once switching from BSP to ASP, we will reduce the mini-batch to be $B$ as in ASP training the batch size is treated as a local value specific to each worker. 
%
We use the \emph{linear scaling rule} for setting the learning rate for training with BSP as $\eta_{BSP} = n\eta$. This is based on prior work that demonstrated the effectiveness of scaling learning rate based on mini-batch size~\cite{goyal2017accurate}.
%
In contrast to prior work that adjusts momentum based on mini-batch size~\cite{lin2019dynamic}, we find that using the \emph{same} momentum value for both BSP and ASP allows \sysname achieve comparable accuracy to training with BSP (i.e., leftmost bar in Figure~\ref{fig:momentum_scaling}). 



\eat{ % much longer version for sigmetrics 
This section describes how to adjust hyper-parameters, which are commonly considered important for training performance~\cite{robbins1951stochastic, senior2013empirical, smith2017don}, for switching between synchronization protocols.
Since our work is not about hyper-parameter tuning, we do not focus on finding the optimal hyper-parameters set for a specific training setting. 
When given the workload and a cluster with a size $n$ for training, we take in an initial set of hyper-parameters, e.g., a mini-batch size of $B$ and a learning rate of $\eta$, as input values provided by the end-user. 
We aim to automatically change the value of these hyper-parameters according to the synchronization protocol used. Our policy requires no manual tuning and optimization for ensuring the performance of synchronization switching. When switching from BSP to ASP, we will scale down the learning rate for ASP as $\eta_{ASP} =\frac{1}{\sqrt{n}}\eta$. This is in large part because the gradient staleness often grows with the cluster size and training with too much staleness can cause divergence that eventually leads to failed training sessions.


\para{Mini-batch size} defines the amount of training workload, e.g., images, per step. To start the training with BSP, we will configure the mini-batch to be $nB$. This configuration is based on both the implementation of BSP batch size in the TensorFlow framework (i.e., as a global value distributed to each worker) and prior work's suggestion of setting BSP batch size proportionally to the cluster size~\cite{goyal2017accurate}. 
We also verify the effectiveness of this configuration empirically, as shown in Figure~\ref{fig:batch_size_scaling}.
Once switching from BSP to ASP, we will reduce the mini-batch to be $B$ as in ASP training the batch size is treated as a local value specific to each worker. 


\para{Learning rate} controls the impact of each gradient batch on model parameter updates. We use the \emph{linear scaling rule} for setting the learning rate for training with BSP as $\eta_{BSP} = n\eta$. This is based on prior work that demonstrated the effectiveness of scaling learning rate based on mini-batch size~\cite{goyal2017accurate}. When switching from BSP to ASP, we will scale down the learning rate for ASP as $\eta_{ASP} =\frac{1}{\sqrt{n}}\eta$. This is in large part because the gradient staleness often grows with the cluster size and training with too much staleness can cause divergence that eventually leads to failed training sessions. Based on our empirical explorations, we found a sub-linear scaling factor of $\frac{1}{\sqrt{n}}$ to be more effective than the linear scaling factor of $\frac{1}{n}$, which caused $\eta_{ASP}$ to be too small and led to slower and worse convergence due to potentially being trapped in saddle points. 

\para{Momentum} is a popular technique in SGD that improves the convergence rate~\cite{rumelhart1986learning} as it helps accelerate SGD in the relevant direction and dampens oscillations of the gradients. In contrast to prior work that adjusts momentum based on mini-batch size to mitigate the negative impact on the training loss~\cite{lin2019dynamic}, we use the same momentum value for both BSP and ASP. Our choice is based on our empirical observation that adjusting momentum when switching from BSP to ASP has very minimal impact on the converged accuracy, as shown in  Figure~\ref{fig:momentum_scaling}. The four methods we explored for setting momentum after switching to ASP are (in order): \1 setting the momentum to 0, \2 setting the momentum to $\frac{1}{n}$ where $n$ is the cluster size, \3 
ramping up the momentum based on $\frac{2^i}{n}$ where $i$ is the number of epochs after switching, \4 ramping up the momentum based on $\frac{i}{n}$ where $i$ is the number of epochs after switching. Both \3 and \4 will stop the ramp up until the momentum reaches the original value used by BSP.
}




==> section/discussion.tex <==
\section{Discussion}

\tian{We should discuss and talk about the potential impacts of adaptive and dynamic SGDs on cloud computing, and potential changes we should make for ML and system sofewares}


\paragraph{How generalizable will the dynamic training configuration work?} 
Given that we only tested a number of cases, it might be useful to discuss if
there is any other configurations that we think might work; and how well they
might work.

% Eval issues 
% PS and worker on same server . PS consumes GPU memory . Fix is ??? 
% Demonstrate feasibility in eval. BSP --> ASP switching once (convergence result not great)
% What are the strenghts of this hybrid approach 
% AWS training service? 
% 

\begin{itemize}
\item Model Synchronization for the cloud. Current ML assumes shared dedicated clusters. Cloud has different performance and interference characteristics, and stragglers can be a bigger problem in many cases. 
\item Need for ML frameworks to be agile in switching between ASP and BSP on the fly (without kill-restart)
\end{itemize}


==> section/eval.tex <==
\section{Evaluation}
\label{sec:eval}

\input{latex-tabs/exp_summary_policies}

We conducted our experiments by training popular deep learning models on Google Cloud Platform (GCP) to quantify \sysname's performance over training exclusively with BSP and with ASP, two commonly chosen baselines~\cite{jiang2019novel,dutta2020slow}. 
% \tian{We could explain briefly why we did not directly compare to SSP and DSSP.}
%
Note, since the performance of existing synchronization protocols all fall in between that of BSP and ASP, we believe evaluating using BSP and ASP provide us a good foundation for understanding \sysname's performance. 
% Performance-wise, prior work reported SSP and DSSP speedup the time-to-accuracy by 1.1X--2X~\cite{zhao2019dynamic} which is lower than \sysname (e.g., see Table~\ref{table:exp_summary_policies}). \shijian{Added this one to state that it's not mutually exclusive} 
Furthermore, semi-synchronous protocols, such as SSP and DSSP, can also be utilized in \sysname (for example switching from SSP to ASP)---\sysname is agnostic to the underlying synchronization protocols. 
% as the two approaches can complement each other.
%
Our evaluation includes systems experiments using our \sysname prototype to evaluate the efficacy of timing policies
% \shijian{Do we need footnote 3 and 4?}\footnote{The evaluation of other two policies: protocol and configuration, were presented in Section~\ref{sec:design}.} 
and framework overhead with real TensorFlow jobs, as well as simulation experiments to analyze the performance and cost of our binary search-based algorithm  under realistic workload conditions. 
Table~\ref{table:exp_summary_policies} summarizes our experiment setups and result highlights. 
% Tian: this result feel like out-of-place.
% We observe that \sysname, achieving up to 4X time-to-accuracy speedup, outperforms the  1.1X--2X speedup achieved by SSP and DSSP~\cite{zhao2019dynamic}.


 
\subsection{Evaluation Setup and Methodology} 
\label{subsec:eval_methodology}

\para{Distributed Training Workloads.} We choose two different workloads, \1 ResNet50 on the CIFAR-100 dataset and \2 ResNet32 on the CIFAR-10 dataset.
% , which allow us to evaluate \sysname's performance on different computational and workload requirements.
Both models are part of the ResNet model family, one of the widely used CNNs for image recognition tasks. We use the ResNet implementations from Tensor2Tensor~\cite{tensor2tensor}.
ResNet50 has more layers than ResNet32, leading to different model parameter size and floating-point operations, and therefore has longer per-batch 
% \tian{per-batch?} \shijian{Per-step here is almost synonymous to per-batch or per-iteration, but for generality's sake per-batch is probably more suitable} 
training time with the same cluster.  
The datasets, each containing 60K images of size 32X32 pixels, are widely used in deep learning research~\cite{cifar10}. The key difference between the two datasets is the number of the classification classes (i.e., CIFAR-100 contains 100 classes vs. CIFAR-10 contains 10 classes); therefore, it often takes more epochs to train on the CIFAR-100. 
%
As such, these two workloads allow us to evaluate \sysname's performance under different computation and learning requirements.


\para{Cluster Setup and Configuration.} 
% We run all experiments on a TensorFlow cluster of 8 (or 16) cloud GPU servers in Google Cloud's \textit{us-west1-b} zone to evaluate \sysname's performance on different cluster sizes~\cite{Or2020-nh,dutta2020slow}. 
We run all experiments on cloud-based GPU clusters in GCP's \textit{us-west1} region; we choose two commonly used cluster sizes of eight and sixteen\footnote{Smaller cluster size has less impact on ASP's converged accuracy~\cite{Li2020-bk}.} to evaluate \sysname's performance~\cite{Or2020-nh,dutta2020slow}.
% \tian{can add why not choose small cluster size} \shijian{smaller-sized clusters don't really suffer as severely in terms of converged accuracy when doing ASP}
Each server, running Ubuntu 18.04 LTS, has 8 vCPUs, 30 GB of main memory, 100GB local HDD storage, and is equipped with one Nvidia K80 GPU card. 
To account for the inherent accuracy variations in SGD-based deep learning training, we repeat each experiment setup five time using the same model parameter initialization algorithm.
% \tian{using the same model parameter initialization algorithm.} \shijian{initialization algorithm, not the actual values}.
We report both the average performance with standard deviation and the runs with the best performance, measured by the highest achieved test accuracy.

\para{Evaluation Metrics.}
We use two groups of metrics for evaluating \sysname's efficiency in parameter synchronization (first group) and its associated overhead (second group).
The first group includes training loss, test accuracy, total training time, and time-to-accuracy. %
\emph{Training loss} is calculated based on the cross-entropy loss function per mini-batch. We report the average training loss collected every 100 ASP steps to avoid incurring excessive measurement overhead~\cite{Li2020-bk}. 
% This measurement frequency is sufficient for our workload, e.g., translating to 9.5 seconds per measurement in the case of ResNet50. In general, the lower the training loss, the higher the test accuracy, the better. 
%
\emph{Test accuracy} refers to the top-1 accuracy of the trained model when evaluating on the test dataset. We measure the test accuracy every 2000 ASP steps on the standalone cluster manager to avoid impacting the training performance. 
A model is said to be converged if its test accuracy has not changed for more than 0.1\% for five evaluations
% \tian{p value?} \shijian{0.1\%} for \tian{Y evaluations.} \shijian{5 evaluations} 
and we report the corresponding value as the \emph{converged accuracy}.
% \tian{How do you determine if the model is converged?} \shijian{when the test accuracy plateaued for a specific amount of iterations} We also report the \emph{converged accuracy} evaluated on the converged model.
% We refer to the test accuracy evaluated on the converged model as \emph{converged test accuracy}, and \emph{converged accuracy} for short. 
%
\emph{Total training time} is the time, including computation and networking time, taken for a training cluster to complete a user-specified workload. We measure this time at the end of each training using the TensorFlow built-in logs. 
% This metric is also a good proxy for comparing throughput and cloud costs. 
%
\emph{Time-to-accuracy (TTA)} denotes the time to reach a specified test accuracy threshold and provides valuable insights into both the training throughput and model accuracy~\cite{coleman2019analysis}. We use the average converged accuracy of models trained with BSP in the same setup as the threshold.
%
For the second group, \emph{search time} quantifies the time for \sysname to find the near-optimal switch timing using the binary search. We calculate search time as the sum of the total training time of all sessions trained during the search. \emph{Switch overhead} describes the total time to switch between synchronization protocols with TensorFlow.

\para{Hyper-parameter Setting.} We set the initial hyper-parameters based on the original ResNet paper~\cite{he2016deep} and use the SGD with momentum of 0.9 as the optimizer. Specifically, we configure the training workload to be 64K steps, batch size to be 128, and learning rate to be 0.1. We use a piece-wise function that decays learning rate at 32K and 48K steps, with scaling factors of 0.1 and 0.01, respectively. Further, we use the configuration policies described in Section~\ref{subsec:hyperparameter} to adjust relevant hyper-parameters based on the specific experiment setup. 


\subsection{Performance of \sysname}
\label{subsec:perf_search_based_policy}

% summarized result 
\input{latex-figs/exp_eval_search_policy_overview}

% detailed result
\input{latex-figs/exp_res32_cifar10_cluster8}
\input{latex-figs/exp_res50_cifar100_cluster8}
\input{latex-figs/exp_res32_cifar10_cluster16}

\subsubsection{End-to-end Comparison}
% \para{End-to-end Comparison.} 
Table~\ref{table:exp_summary_policies} and Figure~\ref{fig:eval_search_policy_overview} summarize the end-to-end training performance achieved by \sysname. In all setups evaluated, \sysname outperforms training exclusively with BSP and with ASP in total training time, TTA, and converged accuracy, respectively. 
For example, we observe that \sysname uses only 19.5\% of the training time while reaching similar converged test accuracy when compared to BSP;
additionally, \sysname improves converged accuracy by 2.5\% with only 1.28X the training time when compared to ASP (exp. setup 1).
The speedups achieved by \sysname are more prominent compared to 1.2-3.7X reported in prior work~\cite{jiang2019novel}; the high-quality converged accuracy is significant as recent innovations on models have similar levels of improvement, e.g., less than 2\%~\cite{gastaldi2017shake, chollet2017xception}.
% when training a ResNet32 on the Cifar-10 dataset using a 8-GPU cluster. 
% \Lijie{The reason is that XXX, as mentioned in Section XX}.
The training speedup comes from \sysname only needs to train a small portion of workload using BSP and the competitive converged accuracy comes from identifying the most appropriate switch timing.
% , as described in Sections~\ref{subsec:ordering} and ~\ref{subsec:offline_binary_search}.
% don't have sapce
% \tian{can add another table comparing to DSSP, TTA: ASP 2993, BSP 6159, SSP 5564, DSSP 3016, accuracy = 0.67}




Furthermore, Figure~\ref{fig:res32_cluster8_eval} details the performance of training a ResNet32 on the CIFAR-10 dataset using an 8-GPU cluster. We plot training loss and test accuracy of the best runs for ASP, BSP, and \sysname in Figures~\ref{fig:res32_cluster8_anytime_loss} and \ref{fig:res32_cluster8_anytime_acc}.
% the best effort run using BSP, ASP, and \sysname, respectively and plot the anytime training loss and test accuracy in Figure~\ref{fig:res32_cluster8_anytime_loss} and Figure~\ref{fig:res32_cluster8_anytime_acc}. 
Interestingly, training with BSP at the first 6.25\% steps allows \sysname to decrease the training loss faster and to lower values (the lower the better), compared to training exclusively with ASP. 
Additionally, even though \sysname does not decrease training loss to the same level as BSP, it still reaches the same converged accuracy. More importantly, \sysname only needs 25\% training time used by BSP to reach the same converged accuracy (i.e., a 4X TTA speedup).
% \footnote{It is worth noting that the time to complete each step varies depending on the synchronization protocols in-use; therefore one cannot directly infer the training time based on the training loss/test accuracy curves (e.g., Figure~\ref{fig:res32_cluster8_anytime_acc}).}.
Further, Figures~\ref{fig:res32_cluster8_converged_acc} and ~\ref{fig:res32_cluster8_training_time} draw the comparison to manual switching, i.e., switching at a static time point, and demonstrate \sysname's utility. 
% , especially at the last learning rate stage \tian{double check}. 
% \shijian{Not sure it is true? Training loss seems to be in-between ASP and BSP at least for resnet32+cifar10, but converged accuracy is on the same level.} 
% \Lijie{The TTA shows that XX, which demonstrates BSP should be used first instead of ASP, as our ordering policy.}


Results of similar magnitude are also observed for the other two setups as shown in Figure~\ref{fig:res50_eval} and Figure~\ref{fig:res32_cluster16_eval}. Note that training ResNet32 with ASP (and training with BSP for less than 50\% steps) in a cluster of 16 GPU servers resulted in failed training due to the training loss divergence. The failed training sessions are likely caused by noisy gradients that are exacerbated with larger cluster sizes. This observation attests to an additional benefit provided by \sysname---being able to complete training in scenarios where ASP cannot. 


% Additionally, using \sysname improves converged accuracy over using ASP by 2.56\% with only 28.5\% training time overhead. Such accuracy improvements are significant as new state-of-the-art models or training techniques often improve the same metric by under 2\%~\cite{gastaldi2017shake, chollet2017xception} and often desirable, especially in the real-world deployment. \shijian{The citations are from new models - not sure if the comparison is apple-to-apple.}
%
% Similarly, training the same workload of ResNet32 on CIFAR10 with a cluster of 16 GPU servers benefits from switching at 50\% workload from BSP to ASP as shown in Figure~\ref{fig:res32_cluster16_eval}. Due to the training loss divergence caused by noisy gradients on a large scale, switching before 50\% (which coincides with learning rate decay) resulted in failed training. Switching at 50\% workload used only 53.6\% of the time for a BSP training session, and reached similar level of converged accuracy of 92.2\% compared to 92.3\% of BSP.
% \shijian{observation on the trend of same workload on different cluster size}


% \para{Summary:} \emph{Our \sysname outperforms two baselines of training exclusively with BSP and with ASP, as well as manual switching, i.e., switching at a static time point.}
 
% \paragraph{Training ResNet50+CIFAR100 on a 8-GPU cluster.} \tian{ground truth comparison}

% \paragraph{Training ResNet32+CIFAR10 on a 16-GPU cluster.} \tian{ground truth comparison}




\subsubsection{Generality Analysis of Our Observations}
% \para{Generality Analysis of Our Observations.} 
% \Lijie{How about changing to this description: our \sysname can work well in different environments: different cluster sizes with different sizes of DL models. Transfer seems that there are some rules for guiding the transferring.}
%
% Next, we analyze how well the policies found by \sysname can be transferred \Lijie{used in different scenarios} to different training scenarios.  
%
\input{latex-figs/exp_cross_compare_policy}
\input{latex-figs/exp_eval_straggler_policies}

Figure~\ref{fig:eval_cross_comp_policy} compares the performance of directly using policies found for the other two setups to the third setup. We make the following key observations. 
First, for similar workloads (i.e., training ResNet32 on Cifar-10 vs. ResNet50 on Cifar-100), the cluster size seems to play an important role in determining the efficiency of the policies. Concretely, training with policy 2 in the experiment setup 1 achieves almost the same converge accuracy (91.7\% vs. 91.4\%) and uses about 33.0\% longer training time. The prolonged training time is expected as policy 2 requires more training to be done with BSP. In comparison, training with policy 3 under the same setup uses 3X of the training time with policy 1.  
% training with policy 3 under the same experiment setup achieved 92.0\% higher\shijian{not sure we can claim it's really higher because it is within the margin of error} test accuracy but with 2.98X times total training time on average. 
Furthermore, by using the correct policy under experiment setup 3, the training successfully finished (without diverging) and achieved comparable test accuracy to using BSP while saving almost 46.4\% training time. As shown in Figure~\ref{fig:res32_cluster16_eval}, training with ASP failed without producing usable models. This observation further suggests the practical utility of \sysname. 


\subsubsection{With Transient Stragglers}



We construct two transient straggler scenarios, mild and moderate, for experiment setup 1 to evaluate the effectiveness of the straggler-aware policies introduced in Section~\ref{subsubsec:online_policies}.
%
In the first scenario, we set the number of stragglers to be 1, the frequency of straggler occurrences to be 1, and inject the slowness by emulating the network latency to be 10ms. 
%
In the second scenario, we increase the number of stragglers, the frequency of straggler occurrences, and the degree of slowness to be 2, 4, and emulated with 30ms network latency. 

Figure~\ref{fig:eval_strag} compares the training performance with and without (baseline) applying our straggler-aware policies. We observe that when the straggler scenario is mild (scenario one), both straggler-aware policies adequately handle the potential performance degradation and even shorten the total training time by 2\%, compared to the straggler-agnostic baseline policy. Furthermore, we find that the greedy policy leads to a 2\% lower converge accuracy while policy two is able to maintain the high-quality converge accuracy. The accuracy degradation is most likely due to having to perform two extra switches, one to ASP and the other back to BSP, before the optimal timing.  
%
Based on our empirical observation, we conclude that the greedy policy does not work in conjunction with \sysname's existing baseline policies.   
%

In contrast, the elastic-based policy is proven to be effective even under moderate levels of slowness. In particular, we observe that this policy not only achieves a similar level of converged accuracy but also leads to a 1.11X speedup. This further suggests that the better course of action is to train without the transient stragglers than to block the remaining cluster nodes from making progress when training BSP.
%

% To evaluate the performance of our proposed policy in an unstable training environment where transient stragglers randomly appear, we conducted two groups of experiments. We define transient stragglers as servers that experience unintentional slowdown due to internal or external issues, and last only for a brief period of time. We consider 4 factors that can contribute to the slowness of stragglers: 1) The duration of the slowness. 2) The frequency that the slowness appears. 3) The number of transient stragglers in a cluster. 4) The individual slowness e.g. network latency on a straggler. 

% For the duration of slowness, we set it to be the total startup time plus termination time of a cloud server on GCE, which is around 100 seconds, found in previous study~\cite{Li2020-bk}. If the slowness of a server is constantly higher than the cost to acquire a new one, it would be more cost-effective to do the latter. 

% For the other factors, we consider two scenarios, where the straggler issue is negligible or severe. In the first scenario the number of stragglers is small (1 straggler), the degree of slowness low (10ms latency), and the frequency the slowness happens is low (happened randomly once before the switching point). In the second scenario, the number of stragglers is larger (2 stragglers), the degree of slowness higher (30ms latency), and the frequency of slowness also higher (randomly happened 4 times before switching).

% We compare our proposed policy (policy 2) to the baseline policy (where no straggler mitigation was applied) and the greedy policy (policy 1). The total training time was measured without the framework switching overhead, quantified in Section~\ref{subsec:practical_overhead}.

% In the first scenario, we can see that policy 1 and 2 can shorten the total training time by around 2\%, proving that the baseline \sysname performance is somewhat resilience to stragglers. However, even with only 1 occurrence of straggler (meaning we have one extra switching back and forth between BSP and ASP) the converged accuracy degraded 2\% compared to baseline and policy 2. Thus the greedy policy is not applicable in practise.

% In the second scenario, we observe that policy 2 can achieve similar level of converged accuracy, while achieving 1.11X speedup. This proves that our proposed policy can effectively reduce impact of straggler on top of the policy applied when no straggler was present.

%TG: we should mention this, but not sure this is the right place to do so.
% Recall that our targeted training workload is repetitive jobs which are very common for deep learning due to its trial-and-error nature \tian{citation.} 


% talk about the implication of the results 
% - random switching policy converges to the expected performance of 50\% switching point

% \tian{should we talk about the 16 GPU servers?} 

% \input{latex-tabs/exp_summary_speedup}

% \subsection{Search-based Policy Overhead Analysis} 

\subsection{Overhead of \sysname}

% \Oren{Can this section be summarized in a few sentences, and the rest of the section moved to the supplement or the ArXiv version?  I think the main point of this section is just that the overhead is small for both the binary search cost and the framework overhead.}

\subsubsection{Binary Search Cost} 
\label{subsec:search_overhead}

% \input{latex-figs/sim_search_cost}
\input{latex-tabs/sim_search_cost_resnet32_8}

% \Lijie{This overhead analysis is too long. We should focus on the performance and accuracy of \sysname compared with other policies. We only need to report the overhead value and then argue if it is acceptable and can be potentially reduced.}


% if the job is recurring, the search cost can be reduced by 12.7/7.7; quite common (seen 
% running BSP once --- no successful settings; if never seen before, the best is to repeat BSP multiple times to get the more accurate ground truth accuracy    
% repeat the candidate runs is often necessary (more likely to see successful settings when repeat more than 3 times), lead to more robust policy 
% with all this combined; new job; bn=3, n =3, search cost is 7.62X 
% m > m * 0.195 + 7.62 -> about 9.5 recurrences (amortization) 

To quantify the overhead of our binary search-based algorithm (in search time) in different training scenarios, i.e., with recurring jobs and fewer measurement runs, we use all our training logs and simulate each search setting 1000 times with the accuracy threshold of 0.01.
% \tian{is it 0.01\% or 0.01? A threshold of 1\% seems to be way too big given the accuracy difference between asp and bsp is only about 3\%.}
%
% Figure~\ref{fig:search_cost_eval} summarizes the normalized search cost to training with BSP for all three experiment setups and 
Table~\ref{table:search_cost_res32} details the cost-performance trade-off (more results are available in our extended report~\cite{syncswitch-extended}). 
%
If the job is recurring, the search cost can be reduced by up to 5X the BSP training.
% ---the exact cost to train with BSP to obtain the target converged accuracy. 
However, when facing a new training job, it is best to at least repeat the BSP runs 3 times. We further observe that with  too few BSP training, the search setting often ends up with significantly lower success probability (e.g., 56.8\% to 82.3\%) in finding the same switching timing as the baseline setting. 
% This suggests the need for repeating measurement given that accuracy can fluctuate.
%

% In short, by using search setting that repeat the BSP and search candidate three times, we can reduce the search cost by 8.1X and 5.1X of the BSP training time for recurring and new jobs, respectively. 
Additionally, we analyze the amortized cost, measured by the number of job recurrences, and the effective training ratio, measured by the multiples of BSP training sessions. The former provides further justification of the cost-effectiveness of our binary search algorithm and the latter signifies the potential information gains. As an example of the search setting (No, 3, 3) in Table~\ref{table:search_cost_res32}, if a job needs to be trained for more than 9 times, a very likely event given the trial-and-error nature of deep learning training, the corresponding search cost is then amortized. Moreover, the search process itself also produces almost 2X valid training sessions compared to training with BSP. In summary, our analysis shows that the search cost is reasonably low and can be further reduced by continuously using \sysname. 

\eat{
In this section, we first quantify the overhead for deriving the switching policies. Recall that when searching for the switching point, \sysname will repeat each configuration five times and leverage the average to decide whether to continue with the search or not. In the case of setup 1, we observe that the search overhead for all experiment setups can be up to 12.71X of training with BSP. This cost can be amortized, calculated by $Cost_{BSP} * m \geq Cost_{switch} * m + Cost_{search}$ where $Cost_{BSP}$, $Cost_{switch}$ and $Cost_{search}$ \Lijie{it is not easy to understand this formula, how about using simple words instead.} denotes the training cost for BSP, solution found by \sysname, and searching process, respectively, and $m$ the times of training. We found if the same job will need to be trained for more than 15 times, a very likely event given the trial-and-error nature of deep learning training. 

Next, we look at the potential of reducing the search cost by reducing the number of runs for each job configuration. 



% \tian{Maybe: set a cost budget based on BSP, analyze the number of eligible ASPs, BSPs, and \sysname performance?}

% \tian{Create a table for the search time needed for training the above-mentioned workloads; put the time overhead in context by comparing to simply training with BSP.}

% \tian{Add the cloud cost analysis to bring out the monetary savings.}

We evaluate the search cost using the algorithm proposed in Section~\ref{sec:design} to search for a near-optimal switching point. We look at two different scenarios under different assumptions: 1) The training workload has been seen before, or a different but similar workload (as analyzed in the previous section) has been trained, so that the target accuracy can be provided as an input. 2) The training workload is unseen, and expected converged accuracy for the model is unknown. 

We run simulated searching process using the data we collected for each training workload and setting as the ground truth. For the first scenario, we set the target accuracy as provided by the historical data. For the second scenario, we conduct BSP training first as the baseline for converged accuracy, and including the cost of BSP training in the total cost for searching. Same as the number of searching, we could use multiple BSP training session to reduce the variance on converged accuracy. But in practice, we found out that converged accuracy for BSP is relatively stable, picking 1 to 5 random data points 100 times in our ground truth data only averaged to a standard deviation of 0.002. Considering the cost of doing BSP is expensive, we compare setting the number of BSP runs $B_n$ the same as the number of searching in one setting with fixed number of 1. For the accuracy delta threshold, we found that either setting it to be the lower-bounded average of the historical data, or 0.01, to be very effective. 

We simulate the searching process with various numbers ($n$ from 1 to 5) of training done for the same setting. We run each simulated searching on workloads 1000 times, and report in Table~\ref{} the total searching cost in comparison to running BSP training 1 time, we also calculate the cost saving since the training sessions inside the searching process can also be seen as effective training sessions in a continuous training environment. Last but not least, we report the success rate as compared to the ground truth of training 5 times for each setting. We define a success to be having the same searching result as the ground truth.
}

\eat{
% this section will be represented in the Motivation/Challenges  
\subsection{Hybrid Synchronization Training Performance}

\eat{\tian{\1 How many runs did we test? \2 The result in Figure~\ref{fig:demo_comp_time} seems to be pretty stable. But how about Figure~\ref{fig:demo_comp_loss} and Figure~\ref{fig:demo_comp_acc}? How much fluctuations? \3 The BSP step and the ASP step correspond to different batch sizes, right? Did not we have discussed an alternative way to plot the results? \4 Still needs a figure for comparing the converged accuracy across different runs. \5 Let's organize relevant figures using subfigures, similar to what we did for previous paper.}}

First of all, we evaluate the effectiveness of synchronization switching in a real world scenario. We trained ResNet32 on CIFAR-10 with a cluster of 8 cloud servers. As shown earlier in section~\ref{sec:design}, we showcase the training performance by starting the training with BSP, then switching to ASP at half the total training epoch. We chose this timing to switch over because it is the first iteration for the searching algorithm, and it also marks the first learning rate decay. We compare the performance to the baselines of using BSP and ASP throughout the training.

\begin{figure*}[t!]
    \centering
    \begin{subfigure}[t]{0.33\textwidth}
        \includegraphics[width=\textwidth]{img/eval_switch_loss.pdf}
        \caption{Comparison of training loss.}
        \label{fig:demo_comp_loss}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.33\textwidth}
        \includegraphics[width=\textwidth]{img/eval_switch_acc.pdf}
        \caption{Comparison of test accuracy.}
        \label{fig:demo_comp_acc}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.33\textwidth}
        \includegraphics[width=\textwidth]{img/eval_switch_time.pdf}
        \caption{Comparison of total training time.}
        \label{fig:demo_comp_time}
    \end{subfigure}
    \caption{\textbf{Training performance comparison for training ResNet32 on CIFAR-10.}}
\end{figure*}

From Figure~\ref{fig:demo_comp_loss}, we observe that the training loss for ASP is extremely noisy compared to BSP, due to gradient staleness. The floor for BSP is also much lower than ASP, meaning that hypothetically, BSP can optimize the loss function for training data better. We can also observe the effect of learning rate decay at around 32k steps, where the training loss sharply decreased especially for BSP. The switching of synchronization caused the training loss to spike up shortly, signaling the worsening of generalization power on training data temporarily. The rise in training loss gradually got brought down, and eventually lower than ASP but higher than BSP. 
Correspondingly, we observe from Figure~\ref{fig:demo_comp_acc} that test accuracy has similar trend as the training loss. ASP converges to worse accuracy than BSP with 1.73\% lower. However, albeit the temporary dip in test accuracy for \sysname, correlating to the training loss spike, we observe the converged accuracy being leveled with BSP baseline, and even 0.9\% higher. 
From both training loss and test accuracy we can also observe that ASP and BSP, especially the latter, didn't really benefit from the second scheduled learning rate decay. On the other hand, both these metrics saw significant improvement after the second learning rate decay in \sysname training.
Figure~\ref{fig:demo_comp_time} shows that ASP finished training the fastest, and is 6.59X faster. \sysname on the other hand is 1.71X faster than BSP, but still 3.85X slower than ASP. 

\paragraph{Summary.} 
% \tian{Where does the proper timing come from? If that is a proper timing, why don't we show the near-optimal switching point? How about the following summary?}
% Synchronization switching at a proper timing can provide training speedup over static BSP, without sacrificing converged accuracy.
% 
Using BSP to start the training and then switching to ASP can lead to various degrees of speedup compared to only using BSP, with minimal impact on the converged accuracy. Our observation suggests the benefit of mixing synchronization and motivates the study of identifying the near-optimal policies. 

% \shijian{Maybe we can also add a new metric Time to Convergence}
% \tian{We should. We also should describe how we determine the convergence.}
}


\eat{
\subsection{Near-optimal switching point searching}

The previously shown result of synchronization switching provided desired training performance improvement. Our next evaluation is on the effectiveness of Algorithm I and how well the found solution transfer to different workload. 


\tian{need to split into two parts: one about the first group of metrics and the other about the overhead.}
We were able to find an near-optimal solution for switching point at 6\% in 5 iterations using Algorithm I. At each iteration the workload percentage was rounded down to the nearest integer. The total time cost for searching is 2.42X of the training time of static BSP. However, as shown in Figure~\ref{fig:optimal_comp_time} the near-optimal solution of switching at 6\% is only 29.6\% slower than static ASP and is 5.13X faster than static BSP. From Figure~\ref{fig:optimal_comp_acc} we can observe that the converged accuracy for optimal SGD switching is comparable to the baseline of static BSP, with only 0.1\% lower. While comparing to static ASP it provides a 2.6\% increase. 

\paragraph{Generalize the solution to similar deep learning jobs.} To consolidate the effectiveness of the found solution, we apply it to similar training jobs and observe the training performance. We trained ResNet50 on CIFAR-100 using \sysname. The results are shown in Figure~\ref{fig:res50_eval}. 


\paragraph{Summary:} The near-optimal switching point could provide further improved training time-accuracy trade-off.

% \tian{It can be confusing to mention that "The total time cost for searching is 2.42X of the training time of static BSP." Is it good or is it bad? Why is it okay to spend the time in searching? \2 How many runs? How generalizable? }

\subsection{Straggler mitigation}
\tian{Important: Maybe we can change the assumption slightly to only focus on the homogeneous training scenario; this in turn allows us to completely remove the evaluation of straggler mitigation.}

With \sysname, the training cluster can adaptively mitigate slowness from workers. We evaluate the straggler mitigation by injecting slowness into a training cluster of 4 cloud servers. To simulate different level of slowness, we add 2 degrees of latency to the target server, with 10 ms and 30 ms respectively. We further add diversity to the straggler scenarios by injecting different number of stragglers of 1 and 2. Since after the switching point \eat{\shijian{we might want to come up with a name: this switching point is based on Alg I or the dynamic policy}} the cluster is already conducting the straggler-resilient ASP training, we inject the slowness before the switching point found in the experiment above.

Figure~\ref{fig:straggler} shows the impact of stragglers on the total training time. \sysname could provide training performance on par with static ASP, which has a slowdown ranging from 5\% to 46\%, and 3\% to 47\%, respectively. On the other hand, static BSP suffers a slowness ranging from 9\% to 174\%.

\begin{figure}[t!]
    \centering
        \includegraphics[width=0.45\textwidth]{img/straggler.pdf}
        \caption{\textbf{Impact of stragglers on training time.} \shijian{PLACEHOLDER: Need a accuracy subplot here for comparison} \eat{\tian{The result does not look very impressive... what is the point of having a different approach, in this case, \sysname, that achieves similar performance as the ASP? \2 Do we have converged accuracy comparison? And how did \sysname compare to ASP in that?}}}
        \label{fig:straggler}
\end{figure}

\paragraph{Summary:} Using the reactive switching policy can completely negate the extra impact of slowness comparing to BSP, and makes it handle stragglers as well as ASP.
}




\subsubsection{Runtime Overhead}
\label{subsec:practical_overhead}

\input{latex-tabs/exp_framework_overhead}
% key takeaways: 
% 1. initialization is needed regardless of \sysname 
% 2. ours is faster than prior work with sequential execution 
% 3. switching once, total framework time can be as low as 3%, which depends on the switching timing and the cluster size 
% (Optional) switching more than once, the switching overhead is on par with just provisioning new workers; 

We quantify the overhead of using \sysname to perform distributed training. Our measurements are based on training ResNet32 on the CIFAR-10 dataset, as the training  framework overhead is largely workload-independent~\cite{Li2020-bk}. Table~\ref{table:framework_overhead} shows the total time spent by \sysname for  initializing the cluster and switching to a different synchronization protocol. 
First, initializing a cluster of twice the workers takes 1.42X the time of initializing a cluster of 8 workers. 
% 128/90 = 1.42
% This observation aligns with prior work which also shows that initialization time can increase slightly with the model size and complexity~\cite{Li2020-bk}. 
Note that one can expect to have similar initialization time even with just the vanilla TensorFlow~\cite{Li2020-bk}. 
Second, by having a configuration actuator that propagates distributed training tasks in parallel, \sysname reduces both the initialization time and switching overhead by 2X and 3.1X, respectively. 
% 157/90 = 1.74, 90/36 = 2.5
% 268/128 = 2.09, 165/53= 3.11
Third, the switching overhead can be as low as 36 seconds, about 1.7\% of the time taken to train the model with \sysname. 
% . This overhead is not only reasonable, being about 1.7\% of the time taken to train the model with \sysname; more importantly, this also translates to two orders of magnitude savings in training time compared to training with BSP. 
% 126/2058.3
% 2058.3/0.2 * 0.8 = 8,233.2 seconds savings 
In summary, \sysname incurs low switching overhead that increases sub-linearly with the cluster size.  
% 53/36 = 1.5X

% Existing popular training frameworks such as TensorFlow and Pytorch do not have built-in supports for turning on and off the synchronization while the training is ongoing. In this section, we quantify the overhead associated with switching between BSP and ASP, as summarized in Table~\ref{table:framework_overhead}. In all setups, the overall switching overhead took less than 12 percent of the total training time. For example, in the case of training Resnet32 on a 8-worker cluster, switching from BSP to ASP took about 36 seconds when switching in parallel and 90 seconds when switching sequentially. In particular, propagating the new synchronization configuration to all cluster nodes took the majority of the time during the switch. Given that \sysname only needs to perform a handful of switches during the entire training process, we feel that the switching overhead is acceptable. 


% %%%
% Due to the lack of native support of at-will switching synchronization during the training, \sysname imposes additional overhead to a training session. In the training performance analysis above, we subtracted the switching overhead to showcase the performance of the switching mechanism itself. In this section, we evaluate the extra overhead of \sysname. 

% In general, the overhead comes from two parts: (1) The controller needs to generate task scripts then propagate to each computing node via TCP/IP protocol. (2) The switching is done by stopping the training, generating model checkpoints, then starting a new training session on the same checkpoint path. To do so, the cluster also needs to be cleaned up of existing long-running parameter server processes, freeing up CPU and GPU memory resources. 

% Sequential execution of the framework controller on a 8-worker cluster to automatically generate scripts and propagate takes 177.671740381 seconds, while parallel execution takes only 43.6758087502 seconds. Checkpoint generation takes only 7.82 seconds on both executions. And the cleaning up takes 14.44 seconds in parallel execution, and 41.43 seconds in sequential execution.
% \tian{add a small table: emphasize \1 overhead vs workload relationship \2 how large overhead in terms of percentage.}

% \paragraph{Summary:} By parallelizing framework threads, we could effectively reduce the system overhead by up to 3.69X.

% \added{Summary Sentence.} To collect data for switching before the 25\% BSP workload mark, we selected 5\% as increment. So we have data for 5\%, 10\%, 15\%, 20\%. For each split we repeated the 3 runs. We trained ResNet32 on Cifar-10, using the total amount of 64k steps with 128 batch size, and piecewise learning rate schedule decaying at 50\% workload and again at 75\% workload with a scaling factor of 0.1. We applied a constant scalar to base learning rate based on what distributed SGD is currently being used, based on previous study and common practise. For BSP we scale it up linearly to the number of workers, and for ASP we scale it down to the square root of the number of workers.

% In general, training loss for 5\% scenarios can reach lower training loss than 4\%. Correlated to this performance, the average test accuracy of 5\% is 0.4\% higher than 4\%, but their margins of error overlap. In comparison, 5\% and 25\% curves reached similar level of training loss, and the resulting test accuracy is different by only 0.15\%. However, the time cost saving from 25\% to 5\% is much larger than 5\% to 4\% (46.5\% faster vs. 4.8\% faster), as expected.

==> section/implementation.tex <==
\section{\sysname Implementation}
\label{sec:impl}

% \tian{Provide an overview of where \sysname stands in the ecosystem.} 

% \tian{Describe components that we implemented to support the dynamic switching policy.} 

% \tian{Describe components that we implemented to support the evaluation of switching policy.}

We built \sysname using Python and shell scripts. The \sysname infrastructure is built on top of the deep learning framework TensorFlow~\cite{tensorflow} with model implementations from Tensor2Tensor~\cite{t2t}, running independently on each node in the training cluster consisted of Google Compute Engine cloud instances. Contrary to the traditional setting of separate servers physically and logically into two categories: \emph{parameter servers} and \emph{workers}, every node serves the roles of both. 
\tian{this is a repetitive paragraph from when we talked about collocated PS in the background. Can be significantly reduced to just what we did and what we plan to do in future work. 
This structure gives us several advantages. Firstly, the increased number of parameter servers can effectively alleviate the communication bottleneck between workers and parameter servers when the latter is significantly less than the former.~\cite{icdcs20,optimus}. Secondly, by getting rid of dedicated parameter servers, we effectively reduced the cost of operation. Last but not least, the model parameters during training are evenly distributed on each nodes, then communicate and update in an N-to-N manner with other nodes. The communication between nodes can be potentially altered into a ring like pattern~\cite{horovod} and further reduce the bottleneck on communication. The potential of dynamically changing the communication pattern during training is left for future work.
}
Since our workload works with moderately sized datasets, each node caches its own copy of the entire training data locally so there's no overhead for loading data repeatedly for each new mini-batch.
% 
% \tian{\1. what is the "infrastructure"? and what is its differences to \sysname? \2 The said benefit to supporting ring-allreduce comes from anything we implemented? Or simply an artifact of using decentralized PS?}
% 

\sysname consists of three main components: Configurator, Cluster Monitor and Decision Maker, as shown in Figure~\ref{fig:sgd_switcher}. 

\begin{figure}[t!]
    \centering
        %\includegraphics[width=0.5\textwidth]{img/implementation.pdf}
        \includegraphics[width=\textwidth]{img/SGD-Switcher-arch.pdf}
        \caption{\textbf{\sysname overview}. Monitor is hooked into the training cluster, arrows omitted for clarity.\Lijie{@Shijian: I have redrawed this figure, you can modify it via img/draw-io/SGD-Switcher.drawio. You can save this drawio file to your disk and reopen it online via http://draw.io}} 
        \label{fig:sgd_switcher}
\end{figure}

Configurator takes in deep learning training jobs from the input user, then sets up the corresponding training configuration taking into regard of factors such as synchronization method used, cluster size etc. The configurator runs on a separate machine outside of the training cluster to save up operation cost. In our case it ran on a local laptop. It is capable of automatically propagating the configured job as different tasks to the computing nodes in the training cluster using \textit{tcp} protocol via \textit{ssh}. Important hyper-parameters are set during this stage. In order to provide more dynamic training configurations, we instrumented customized hook functions in TensorFlow running on each node. The hook functions can achieve a wide range of utilities such as dynamically changing hyper-parameters such as momentum during training, as well as outputting training metrics to the Cluster Monitor. 

\tian{the mentioned of external events might need to be removed
Cluster Monitor actively checks the status of the training clusters for external events such as the emergence of stragglers.
}It keeps check on internal training events such as the magnitude of gradients etc. The Cluster Monitor is powered by an RPC server running independently to the training cluster. To save operation cost, we collocate the monitor on the evaluator node in the cluster, who runs evaluation on the trained model to get test accuracy. Thus the Cluster Monitor also collects and keeps a consistent training path for the given training job.

The Decision Maker takes input metrics on both external and internal events of the training, and modify the next stage of the job according to switching policy as discussed in section~\ref{sec:design}, which are light-weight scripts that are pluggable to \sysname. The new stage for the job will feed back to the Configurator as a training job iterating on top of an existing one, and be propagated to all the computing nodes in the training cluster.
% 
% \tian{The policies refer to the switching policies, right? We should put a backward reference to the Design section to indicate all the policies we implemented.}
%
% \tian{what does "new job" refer to? the user submitted or \sysname submitted?}
%

To ensure that the synchronization switching can be properly triggered in the event-driven policies, we implemented several hook functions in \textit{TensorFlow}. The hook functions actively collect and check the internal metrics either from \textit{TensorFlow} logs or the compute graph for selected metrics such as training throughput and training loss. The values of these metrics are then fed back to the monitor for analysis and processing.

As the current deep learning frameworks don't support changing synchronization while keeping the training going, we adopted the workaround method of restoring training sessions from checkpoints. When a switching decision is made to change the synchronization method, we stop the on-going training session and \tian{note that to further reduce model checkpoint overhead, we can just wait to switch until the next checkpoint---but this does not seem to be taking too much of times comparatively.
generate the latest model checkpoints.
}
Then we resume from these checkpoints with a new training session with modified training configurations. Due to this lack of support for dynamic switching from the framework, each time we switch synchronization there's extra overhead incurred onto total training time. We instrumented timer functions in training sessions to both collect raw training time and training time without the aforementioned overhead. 


==> section/intro.tex <==
\section{Introduction}

% Introduction structure
% \shijian{Five-paragraph structure: 1. Stating the broad problem. In our case it's the distribute training performance optimization. 2. Narrow down the problem to the synchronization of workers. Stating why the existing solution needs to be improved. 3. Present and demonstrate our work and ideas. 4. State why our work is different than related. 5. Roadmap of the paper.}

Deep neural networks (DNNs) are powerful machine learning models that have gained massive popularity in various areas such as computer vision or natural language processing. However, training DNNs can be time and resource consuming. Thus optimizing training performance has been an active area in research. \Lijie{To delete: One popular technique to speedup the process is to use multiple computing nodes to perform distributed training.} Distributed training of deep neural networks mainly consists of two iterative procedures. 
\tian{is the following two-steps per distributed training or per PS-based distributed training?}
First, many workers compute new parameters \tian{parameters or gradients?} from the training data in parallel using popular optimization algorithms such as stochastic gradient descent (SGD). \Lijie{This step can be accelerated by increasing the parallelism (i.e., using more nodes)}. In the second step, the newly generated model parameters will be aggregated from all workers and processed \tian{how?} in preparation of parameters for the next iteration.  \Lijie{This step needs parameter synchronization protocols to perform the aggregation-update.}
% TG: rewrote the following and please double check the meaning.
% (1) computing new parameters from training data, which is usually performed on many workers in parallel using SGD-based algorithms. (2) updating parameter, which collects the computed parameters from workers and compute the new ones for next iteration.


% Deep neural networks (DNNs) are powerful machine learning models that have gained massive popularity in various areas such as computer vision or natural language processing. The training of deep neural networks relies on almost exclusively on mini-batch stochastic gradient descent (SGD) based algorithms for optimization, \Lijie{which is usually parallelized by data parallelism (i.e., data are partitioned into different nodes, while the parameters are updated and synchronized by parameter synchronization protocol. }
% However, training DNNs needs enormous amount of computing power and time to reach convergence. Facing the increasingly resource demanding tasks of training deep neural networks, researchers have been utilizing parallelism to speed up the training process, in order to save the cost of training. SGD-based algorithms are inherently serial, thus parallelism in deep learning usually focus on either parallelizing the model or the training data on multiple nodes, optimized by what is called distributed SGD. \tian{the first and second paragraphs should be condensed to one and mainly focused on motivating the need and benefits provided by distributed training.} \shijian{Done: condensed and restructured a little}


\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{0.38\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/intro.pdf}
        \caption{Current synchronization protocols.
        }
        \label{fig:sync-compare}
    \end{subfigure}
    \qquad
    \begin{subfigure}[t]{0.56\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/BSP-ASP-Compare.pdf}
        \caption{Comparison between BSP and ASP.}
        \label{fig:bsp-and-asp-demo}
    \end{subfigure}
    \caption{Two popular distributed parameter synchronization protocols. When using BSP, PSs employ a barrier for gradient collection and only start to update parameters once all gradients are aggregated. In contrast, when using ASP, individual worker pushes gradients and pulls parameters at their own paces.} 
    \label{fig:distributed_synchronization_protocols}
\end{figure}

% \begin{figure}[t!]
%     \centering
    
%         \includegraphics[width=0.45\textwidth]{img/intro.pdf}
%         \caption{\textbf{Comparison of parameter synchronization protocols.} Commonly used protocols such as ASP and BSP exhibit distinct advantages in either training throughput and converged test accuracy. Existing work often focus on balancing the trade-offs while our proposed solution \sysname can improve the training throughput without satisfying the converged accuracy, compared to BSP. 
%         \tian{figure: x-axis and y-axis labels should be centered; "Training Throughput" is better to be vertical; is it possible to make the left bottom part look less empty...; is it better to add some citations to inside the circle?}
%         % TG: rewrote the following and please double check the meaning.
%         % \textbf{Parameter synchronization protocols and their associated performance characteristics.} Studies have been done to devise new synchronization protocols with trade-offs between converged accuracy and training throughput. \sysname could potentially achieve similar level of training throughput while maintaining the converged accuracy at BSP level or better.
%         }
%         \label{fig:intro}
% \end{figure}

Traditionally, there are two parameter synchronization protocols in the phase of updating parameters: Bulk Synchronous Parallel (BSP) and Asynchronous Parallel (ASP).
% TG: very little information gain
% , each more suitable to handle a different scenario, with different trade-offs.  
BSP deploys full synchronization among the nodes in each iteration to update model parameters, boasting low loss and good converged accuracy, \Lijie{This protocol is used by Tensorflow and XX by default,} but is prone to straggler problem. ASP updates the model parameters whenever a node finished a mini-batch, allowing worker nodes to work at their own pace, thus alleviated from straggler problem. \Lijie{This protocol can be used in XX}. However, due to the use of stale gradients on some workers, the potential converged accuracy for ASP is generally worse than BSP. It is hard for both users and deep learning frameworks to determine the best parameter synchronization protocol, since both the convergence curve and stragglers are unpredictable and dynamically changing. 
%
\tian{we should give examples of a category of work instead of picking out a particular work for analyzing its weakness.}
Previous researchers have designed \Lijie{several optimized} synchronization protocols. One is semi synchronization protocol like SSP. However, this protocol introduce extra hyper-parameter like \textit{staleness}, which is static and hard to determine for users. Another is XX.
%
\tian{needs discussion: is it better to have Figure~\ref{fig:intro} here? The rationale unpredictable, dynamic, and static all feel quite confusing to me.}

In this work, we make the first attempt to simultaneously improve the training throughput (i.e., shorten total training time) and the converged test accuracy, in contrast to trading-off one for the other as in prior work \tian{add citation}. 
\tian{We should describe the challenges we need to solve in devising our solutions; such as costly to sample the training performance and the inherent variation of SGD etc. Maybe we can add it here.} 
\Lijie{Our main idea is to adaptively switching (choosing the best) parameter synchronization protocols during distributed training, in order to balance the training throughput and convergence rate. However, there are many research problems and challenges:

(1) Does this switching synchronization protocol work (improve the performance or convergence rate)? Why it works? Using one paragraph to describe the related challenges and our solutions. We first performed an empirical study on XX.
(2) How to switch? from BSP to ASP or from ASP to BSP. Switch once or many times? We design a set of policies XX.
(3) When to switch? We empirically XX. Based on XX, we designed XX.}

To address the abovementioned challenges, we leverage both empirical observations and theoretical analysis to devise a set of policies that govern the use of synchronization protocols during distributed training.
\tian{Our key insight is: maximize the time the workers are spending on training asynchronously while still providing the convergence guarantees!}
More specifically, we quantify and explore the potential benefits of adaptively choosing parameter synchronization protocols during distributed training. We experimentally compare performance differences when training popular deep learning models and image datasets, with different synchronization protocols. Our empirical observations reveal two key insights. First, for a given workload, training it first with the BSP and then switching to ASP often result in noticeable training time reduction. 

Second, the additional amount of time we need to spend in training the model with BSP is not necessarily proportional to the final converged accuracy gain \Lijie{This sentence is hard to understand}. Centered around these two insights, we further reduce the initial problem to determining the appropriate timing to start training with ASP. We develop two different approaches, one is based on empirical search and the other is based on the internal training state, for finding the near-optimal switch point that can greatly speedup training while keeping the converged accuracy high. 
\tian{Not sure if we need this anymore: We further improve the robustness of distributed training performance by monitoring the external training environment and triggering the use of ASP upon detecting stragglers.} 
We implement a prototype of \sysname on Tensorflow and Tensor2Tensor. Experimental results showed that \sysname \tian{result highlights ideally should cover speedup, accuracy, generality, and overhead.}

Our work differs from previous studies in that our work takes a minimalist approach of mixing existing synchronization protocols instead of devising new ones. This gives our method better extensibility to be applied to more than just our selected protocols. In the previous work, efforts were made to find better trade-offs between training time and converged accuracy. Figure~\ref{fig:intro} shows that our work can achieve similar level of training throughput as other work, while improving on the metric of converged accuracy. Additionally, our proposed method doesn't introduce new hyper-parameters, which in themselves are hard to tune. 

% TG: I tried to be more directly when describing exactly what we did and why we did it; instead of doing too much setup. I feel that raising a question without providing a solution is a bit too susp
% \eat{specifically the synchronization methods of the nodes, to exploit the advantages of different
% configurations, or to adapt to the changes in the cloud environment.} 
% %
% Our key goal is to shorten the total training time to complete a given workload, making convergence reached earlier, while maintaining good converged accuracy. To achieve this goal, We design smart switching policies, which solve three problems. (1) does switching improve the performance? Our study showed that switching can in fact maintain or even improve upon the converged accuracy of BSP. (2) how to switch? We proposed discovered simple rules to conduct switching in proper order (3) When to switch? We proposed several policies to find the near-optimal solution that can greatly speedup training while keeping the converged accuracy high. We implemented the prototype on Tensorflow and Tensor2Tensor. Experimental results showed that our approach could \shijian{a decisive conclusion here}.


% \Lijie{Our targeted environment? Static cluster of dynamically changing cluster? homogenous cluster or heterogenous cluster?}

% Traditionally, distributed training assumes a static training environment, e.g. the training configurations and most hyper-parameters don't change during the entire training session. Furthermore, as we factor the cloud environment into training DNNs, which is one of the most popular platform for deep learning at the moment, there's no guarantee that the computing notes would stay with stable performances or even a constant amount of nodes, due to geographical separation, unreliable networks, pricing or resource contention on the physical servers. 

% \tian{Too much padding before this paragraph and we should not wait this long to telling the reader what this paper is about...} \shijian{With the modifications it still seems to be too much padding? But we need to introduce the ideas of distributed SGD assuming the reviews don't really know much about what we are talking about} \tian{No really. Introduction is not the place to go into details and provide background. We should focus on laying out the arguments of why it is important to look at the problem and why our approaches are effective.} \shijian{actually getting rid of all the comments would land this much earlier in the section}


% In this work, we make the first attempt to explore the potential benefits of
% switching the training configurations during training, specifically the
% synchronization methods of the nodes, to exploit the advantages of different
% configurations, or to adapt to the changes in the cloud environment. Our goal is to shorten the total training time to complete an amount of workload, making convergence reached earlier, while maintaining good converged accuracy. \Lijie{We design XX switching policies, which contains how to switch (from ASP to BSP or from BSP to ASP), when to switch,    Furthermore, our method should be robust to the unstable training environment.
% \tian{motivates the need for dynamic SGD switching, provide intuition of why it might work, and give evidence that it actually worked in our tested conditions.}

\begin{figure}[t]
    \centering
        \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/intro_intuition.pdf}
        \caption{Training Time}
        \label{fig:intro_comp}
        \end{subfigure}
        \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/intro_intuition_2.pdf}
        \label{fig:intro_comp_2}
        \caption{Converged Accuracy}
        \end{subfigure}
    \caption{\textbf{Comparison of SGD switching to ASP and BSP} SGD switching achieved similar converged accuracy to BSP, while greatly reduced training time. \tian{Please fix the figure formats based on previously discussed guidelines. Also, this figure does not seem to be referenced? What is a good place to reference?}}
\end{figure}

% Prior work for efficient distributed training \tian{mentions a few
% categorizations, like what we did for Perseus}. 
% \shijian{need to create a visualization or table of different distributed training optimization techniques, and how ours is in an area that no one has tackled}
% Our work complements these existing works by providing the basis and argument
% for dynamic training environment. 

% \Lijie{How about listing the research questions? 1. study: the effects of switching? the root causes. 2. when to switch? 3. how to switch?} \shijian{research questions were listed in a later section}

We make the following contributions: \tian{Did not read these bullet points. We have to come back here}

\begin{itemize}
\item Our proposed \sysname policies simultaneously improve the training throughput while maintaining high-quality test accuracy. These policies can be used for distributed training and have been evaluated under the Parameter server-based architecture. 
\item{We are the first in hybridizing different synchronization methods to achieve training performance improvement. By mixing existing synchronization techniques we can take the best of both worlds, speeding up distributed training while maintaining the model accuracy}
\item{We integrated different policies and strategies to deal with different training scenarios, both in terms of internal training performance and external training environment}
\item{We identified and tuned several key training hyper-parameters to prevent the training performance with hybrid synchronization to degrade. At the meantime, we avoid introducing new hyper-parameters to further complicate the training configuration}
\item We evaluated the proposed method with real world workload \tian{TODO}
\end{itemize}



The rest of the paper is organized as follows: In the next section, we will talk about the backgrounds. In section III, we introduce the methodology we conduct the experiments, and the policies for switching. In section IV, we demonstrate the design principles of switching policies. In section V, the implementation of \sysname is introduced. We evaluate the performance of \sysname and compare it to baselines in section VI. In section VII we discuss related work. In the last section we draw some conclusions and outline the future work.
